Modular and Submodular Optimization with Multiple Knapsack Constraints via Fractional Grouping

A multiple knapsack constraint over a set of items is defined by a set of bins of arbitrary capacities, and a weight for each of the items. An assignment for the constraint is an allocation of subsets of items to the bins which adheres to bin capacities. In this paper we present a unified algorithm that yields efficient approximations for a wide class of submodular and modular optimization problems involving multiple knapsack constraints. One notable example is a polynomial time approximation scheme for Multiple-Choice Multiple Knapsack, improving upon the best known ratio of $2$. Another example is Non-monotone Submodular Multiple Knapsack, for which we obtain a $(0.385-\varepsilon)$-approximation, matching the best known ratio for a single knapsack constraint. The robustness of our algorithm is achieved by applying a novel fractional variant of the classical linear grouping technique, which is of independent interest.

==> constant.tex <==

In this section we present an approximation algorithm for $d$-MKCP instances.
%The algorithm leverages the block polytope from Section \ref{sec:block} along with several additional techniques.
The algorithm follows a common scheme of enumeration, continuous optimization and rounding used in previous works~\cite{FC84,CVZ10,KST13,FKNRS20}.
The novelty of our algorithm lies in the 
Fractional Grouping technique of Section \ref{sec:grouping} and in an innovative Block Association technique.
%The novelty of our algorithm lies 
%in the application of Fractional Grouping 
%in the block polytope representation of Section \ref{sec:grouping} 
%(extended to general MKC constraints)
%polytope representation
%of a $d$-MKS constraint, extending the 
% and in using an innovative 
 % Block Association procedure. 
% The novelty of the algorithm lies in %the combination of the techniques 
%the block polytope from Section \ref{sec:block} 
 %and in an innovative {\em block association} procedure. 
Both techniques are employed mainly
%mostly encapsulated
 within a  $\pack$ procedure which
finds an assignment for a randomly sampled set of items.
%
%alongside the two novel procedures: the $\pack$ procedure (which follows from Lemma \ref{lem:second_creteria} of Section \ref{sec:block}) and the block association procedure. 
We first give an overview of the algorithm and used techniques. The $\pack$ and 
Block Association procedures are described in Section~\ref{sec:packing}.

%We say $\II\subseteq 2^I$ is a {\em valid constraint} if $\II=2^I$, $\II$ is an independent set of a matroid or a matroid intersection, or $\II$ is a matching.
Recall that $d$-MKCP is defined in Section \ref{sec:prob_def}, along with the definition of a valid constraint, $\II$, and a valid pair $(\II,f)$ of a constraint and a function. 
Let $\mathcal{T} = \left(I, \left( \mathcal{K}_t\right)_{t=1}^d, \II, f \right)$ be a $d$-MKCP instance, where $\mathcal{K}_t = (w_t, B_t, W_t)$, $1\leq t\leq d$ are the $d$ multiple knapsack constraints. 

The algorithm leverages submodular concentration bounds (e.g., \cite{Vo10}), along with elimination of a constant number of items from an optimal solution. To preserve the approximation ratio, both techniques require that the marginal value of items, $f(\{i\})-f(\emptyset)$, is small. As the input instance does not necessarily satisfy this requirement, an enumeration phase is used to obtain a {\em residual instance} for which the requirement holds.

%The enumeration iterates over all subsets $S\subseteq I$ of bounded size and (disjoint) assignments of $S$ into the $d$ MKS. 

 %Let $S^*\subseteq I$ be an optimal solution for a given instance. For any constant $\xi\in\mathbb{N}$ there exists a subset $S\subseteq S^*$  such that $|S|\leq \xi$ and for any $i\in S^*\setminus S$ it holds that $f_S(\{i\})= f(S\cup\{i\})-f(S)  \leq \frac{OPT}{\xi}$.  
 
 %Note, there is a polynomial number of such subsets $A$ (and their different assignments to $B$). Thus, our algorithm enumerates overall possible partial assignments and completes it into a solution for $\mathcal{T}$. The best solution is selected from the set of constructed solutions. As we are guaranteed to iterate over set $A$ and its assignment, it is enough to find a solution for the residual problem.

The {\em residual instance} is formally defined as follows.
Let $S$ and $(A_t)_{t=1}^{d}$ be a solution of $\mathcal{T}$,
and let $\xi\in \mathbb{N}$. We define the residual instance of $\mathcal{T},S,(A_t)_{t=1}^d$ and $\xi$ as the
$d$-MKCP instance $\mathcal{T}'=\left(I', \left( \mathcal{K}'_t\right)_{t=1}^d,  \II', g \right)$, where
\begin{enumerate}
	\item
	$I'=\left\{ i\in I\setminus S ~\middle|~ f(\{i\}\cup S )-f(S)\leq \frac{f(S)}{\xi}\right\}$.
	\item The function 
	$g:2^{I'}\rightarrow \mathbb{R}_{\geq 0}$ is defined by $g(T)=f(S\cup T)$.
	\item For any $1\leq t\leq  d$, $\mathcal{K}'_t = (w_t, B_t, W'_t)$, where $W'_t(b)= W_t(b) - w_t(A_t(b))$ for all $b\in B_t$.
	\item
	$\II' =\{ T\subseteq I'~|~T\cup S \in \II \}$. 
\end{enumerate}

We note that the function $g$ is non-negative and submodular. Furthermore (as shown in Lemma~\ref{lem:submodular_cup}), $g$ is monotone (modular) if $f$ is monotone (modular).
%We note that function $g$ preserves modularity, submodularity, monotonicity and non-negativity properties of $f$ 
%(see Lemma \ref{lem:submodular_cup}). 
Also, if $\II$ describes a constraint (matroid, matroid intersection or matching constraint), $\II'$ describes a constraint of the same type. That is, both $\II'$ and the pair $(\II',g)$ are valid.  
If $T\subseteq I'$ and its assignment $(D_t)_{t=1}^{d}$ define a solution for the residual 
instance $\mathcal{T}'$, then it can be easily verified that $S\cup T$ and $(A_t \cup D_t)_{t=1}^{d}$  are a solution for the original instance $\mathcal{T}$.\footnote{Given two assignments $A_1,A_2:B\rightarrow 2^I$, we define $D=A_1 \cup A_2$ by $D(b)=A_1(b)\cup A_b(b)$ for all $b\in B$.} Furthermore, by definition, $f(S\cup T)=g(T)$.

%The marginal value of items in an residual instance is bounded due to the definition of $I'$. The 
The next lemma states that the residual instance
with a specific solution preserves the optimum.\footnote{Given an assignment $A:B\rightarrow 2^I$ and a set $S\subseteq I$, we define $A\cap S$ ($A\setminus S$) to be the assignment $D:B\rightarrow 2^I$ such that $D(b)=A(b)\cap S$ ($D(b)=A(b)\setminus S$) for every $b\in B$. }
\begin{lemma}
	\label{lem:residual_generic}
	Let $\xi\in \mathbb{N}$, $\mathcal{T}$ be an instance of $d$-MKCP, and $S^*$,$(A^*_t)_{t=1}^d $ a (possibly optimal) solution for $\mathcal{T}$. Then there is  $S\subseteq S^*$, $|S|\leq \xi$  such that $S^*\setminus S$ and $(A^*_t\setminus S)$ is a solution for the residual instance of 
	$\mathcal{T}$,  $S$, $(A^*_t\cap S)_{t=1}^{d}$ and $\xi$.
\end{lemma}
The proof of the lemma is standard in submodular optimization. For completeness, we give it in Appendix~\ref{app:sub_prop}.
The enumeration (Step \ref{constant:loop}) of Algorithm \ref{alg:constant} iterates over all subsets $S'\subseteq I$, $|S'|\leq \xi$ and disjoint assignments\footnote{An assignment $A:B\rightarrow 2^I$ is disjoint  if for any $b_1, b_2\in B$, $b_1\neq b_2$ it holds that $A(b_1)\cap A(b_2)=\emptyset$.} 
	$(A_t)_{t=1}^{d}$ of $S'$ to the $d$ MKCs, and finds an approximate solution for each residual instance. The number of  possible subsets and assignments is polynomial for a fixed $\xi$. In one of these iterations, $S'=S$ and $A_t=A^*_t\cap S$ for every $1\leq t\leq d$ ($S$ is the set from Lemma \ref{lem:residual_generic}). In this specific iteration, the value of the optimal solution for the residual instance equals to the value of the optimal solution for the original instance; thus, the approximate solution for the residual instance can be used to derive an approximate solution for the input instance.

In \cite{FKNRS20} the authors showed how an MKC can be converted into an  {\em $N$-leveled} constraint.
%Given a single MKS instance it was show by \cite{FKNRS20} how to convert it into an {\em $N$-leveled} instance. 
In such constraints the set of bins $B$ can be partitioned into blocks which adhere to a specific structure.

\begin{definition}
	For any $N\in \mathbb{N}$, a set of bins $B$ and capacities $W:B\rightarrow \mathbb{R}_{\geq 0}$,  we say that a partition $(K_j)_{j=0}^\ell$ of $B$
	is {\em $N$-leveled} if, for all $0\leq j \leq \ell$, $K_j$ is a block and  $|K_j|= N^{\floor{\frac{j}{N^2}}}$. 
\end{definition}

Algorithm~\ref{alg:constant} converts each of the $d$ MKCs into an $N$-leveled constraint. 
The $N$-leveled constraints are useful as each block can be represented separately by a block polytope (see Definition \ref{def:block_polytope}). Furthermore, the fact that the number of bins per block is increasing is crucial for the success of the subsequent sampling process. We note that these two properties were similarly exploited in \cite{FKNRS20}. The following lemma, adapted from~\cite{FKNRS20}, shows that any MKC can be converted into an $N$-leveled constraint with only a small decrease in the value of an optimal solution. %Since the number of MKS, $d$, is constant, each MKS can be converted separately.

\begin{lemma}
	\label{lem:structuring}
	For any $N$, set of bins $B$ and capacities $W:B\rightarrow \mathbb{R}_{\geq 0}$, there is $\tilde{B}\subseteq B$,  capacities $\tilde{W}:\tilde{B}\rightarrow \mathbb{R}_{\geq 0}$,
	and an $N$-leveled partition  $(\tilde{K}_j)_{j=0}^\ell$ of $\tilde{B}$,
	such that
	\begin{enumerate}
		\item $\tilde{B}$, $\tilde{W}$ and $(\tilde{K}_j)_{j=0}^\ell$ can be computed in polynomial time.
		\item
		The bin capacities satisfy $\tilde{W}(b) \leq W(b)$, for every $b\in \tilde{B}$.
		\item
		\label{structuring_prop2}
		For any set of items $I$, weight function  $w:I\rightarrow \mathbb{R}_{\geq 0}$, a subset $S\subseteq I$ feasible for the MKC $(w,B,W)$ over $I$, and a submodular function $f:2^I \rightarrow \mathbb{R}_{\geq 0}$, there is  $\tilde{S}\subseteq S$ feasible for the MKC $(w,\tilde{B},\tilde{W})$ such that $f(\tilde{S}) \geq \left(1- \frac{1}{N}\right) f(S)$.\footnote{We say $S$ is feasible for a MKC $(w,B,W)$ if there is a feasible assignment $A$ of $S$ w.r.t to $(w,B,W)$.}
	\end{enumerate}
	We refer to $\tilde{B}$ and $\tilde{W}$ as the $N$-leveled constraint of $B$ and $W$. 
\end{lemma}

The proof of the lemma requires a minor adaptation of the proof in~\cite{FKNRS20}.  
We provide the proof in Appendix~\ref{sec:structuring} for completeness. 

Algorithm~\ref{alg:constant} relies on  finding an approximate solution $\bx\in [0,1]^I$ for the multilinear optimization problem (defined in Section \ref{sec:related}), and subsequently rounding $\bx$ to a set $R\subseteq I$.
To utilize existing  algorithms for the multilinear problem, we represent an MKC as a polytope. 
Consider an MKC $(w,B,W)$ converted by the algorithm into an $N$-leveled constraint. Let $\left(K_j\right)_{j=0}^{\ell}$ be a partition of $B$ into blocks. 
In the following we give a representation of the MKC by a polytope where each block is 
represented by its  block polytope.

\begin{definition}
	\label{def:extended_gamma_partition}
	For $\gamma>0$, the  extended $\gamma$-partition polytope of $(w,B,W)$ and $\left(K_j\right)_{j=0}^{\ell}$ is
	\begin{equation}
	\label{eq:ex_gamma_partition}
	P^e= \left\{ (\bx, \by^0, \ldots, \by^\ell)~\middle|~ \begin{array}{lcc} &\bx \in [0,1]^I&~~ \\  \forall  0\leq j \leq \ell:& \by^{j}\in P_{K_j} &\\ & \sum_{j=0}^{\ell} \by^j = \bx&\\
	\forall 0\leq j \leq \ell, |K_j|=1, i\in I \setminus L_{K_j, \gamma }:& ~\by^j_i=0&
	\end{array}
	\right\}
	\end{equation}
	where $P_{K_j}$ is the block polytope of $K_j$ (see Definition \ref{def:block_polytope}).  
\end{definition}
The last constraint in \eqref{eq:ex_gamma_partition} prohibits the assignment of  $\gamma$-heavy items to blocks with a single bin.  It can be viewed as analog to the elimination of large items  in \cite{KST13}. As the number of blocks with a single bin and the value of each item in the residual instance are bounded, the removal of all $\gamma$-heavy items from a solution incurs a bounded decrease in value. 

The polytope used in the multilinear optimization problem is a projection of \eqref{eq:ex_gamma_partition}.
\begin{definition}
	For $\gamma>0$, the $\gamma$-partition polytope of $(w,B,W)$ and $\left(K_j\right)_{j=0}^{\ell}$ is
	\begin{equation}
	\label{eq:gamma_partition}
	P= \left\{ \bx  \in [0,1]^I~\middle|~ \exists \by^0,\ldots \by^{\ell} \in [0,1]^I \text{ s.t. } (\bx, \by^0, \ldots, \by^\ell) \in P^e~\right\}
	\end{equation}
	where $P^e$ is the extended $\gamma$-partition  polytope of $(w,B,W)$ and $\left(K_j\right)_{j=0}^{\ell}$.
\end{definition}


It should be noted that $-$ excluding the requirement that no $\gamma$-heavy items can be assigned to blocks of a single bin $-$ the partition polytope is sound for the problem.
% \ariel{hadas, please verify "up to" is properly used here}.
%Modified --H
\begin{lemma}
	\label{lem:gamma_soundness}
	Let $(w,B,W)$ be an MKC, $(K_j)_{j=0}^{\ell}$ a partition of bins to blocks and $\gamma>0$. Also, let 
	$A$ be a feasible assignment for $(w,B,W)$ such that, for any  $0\leq j \leq \ell$  for which $K_j=\{b\}$,  it holds that $A(b)\subseteq L_{K_j, \gamma}$.
	 Then $\one_S \in P$, where  $S=\bigcup_{b\in B} A(b)$ and $P$ is the $\gamma$-partition polytope of $(w,B,W)$ and  $(K_j)_{j=0}^{\ell}$.
\end{lemma}

Let $P(\II')$  be the convex hull of $\II'$, and and let $P_t$ be the $\gamma$-partition polytope of the $t$-th MKC (of the $N$-leveled residual instance). 
Algorithm~\ref{alg:constant} 
uses the polytope $P=P(\II') \cap \left( \bigcap_{t=1}^d P_t\right)$ to represent the instance. 
As in the case of the block polytope, while 
$\max_{\bx\in P} \bc \cdot \bx$ cannot be solved exactly in polynomial time, it can  be approximated, as stated in the next lemma.
\begin{lemma}
	\label{lem:gamam_partitionpoly_fptas}
	Given $d$ MKCs $(w_t,B_t,W_t)$ and a partition $\left(K^t_j\right)_{j=1}^{\ell_t}$ of the bins   $B_t$ to blocks for $1\leq t\leq d$,  $\gamma>0$, a valid constraint $\II$ and a vector $\bc\in \mathbb{R}^I$, let $P_t$ be the $\gamma$-partition polytope of $(w_t, B_t, W_t)$ and $\left(K^t_j\right)_{j=1}^{\ell_t}$, and 
	 $P=P(\II) \cap \left( \bigcap_{t=1}^d P_t\right)$. Then there is an FPTAS for the problem of finding $\bx \in P$ such that $\bx \cdot \bc$ is maximized.
	%$P_K$ is approximable. 
\end{lemma}
 The lemma follows from known techniques for approximating an exponential size linear program using an approximate separation oracle for the dual problem, as in the case of Lemma~\ref{lem:poly_fptas}. We give the proof in Appendix~\ref{app:poly_fptas}. 


Algorithm~\ref{alg:constant} finds a fractional solution $\bx\in P(\II') \cap \left( \bigcap_{t=1}^d P_t\right)$ such that $G(\bx)$ approximates the optimal solution ($G$ is the multilinear extension of  $g$, the value function of the residual instance). This can be done using the Algorithms of~\cite{BF19, CCPV07}, or 
Lemma~\ref{lem:gamam_partitionpoly_fptas}, depending on whether $g$ is non-monotone submodular, monotone submodular, or modular.




The fractional solution $\bx$ is rounded into an integral solution. The rounding procedure starts by sampling a random set of items $R\in \II'$ such that $\Pr(i\in R) = (1-\delta)^2 \bx_i$. The technique by which $R$ is sampled depends on $\II'$. If $\II'=2^{I'}$ then $R$ is sampled according to $\bx$, i.e., $R\sim \bx$ (the distribution is defined in Section~\ref{sec:related}). If $\II'$ is a matroid constraint, the sampling of \cite{CVZ10} is used. Finally, if $\II'$ is a matroid intersection, or a matching constraint, then the dependent rounding technique of \cite{CVZ11} is used. We note that the last two techniques are often referred to as {\em Randomized Swap Rounding}. While each sampling method is slightly different, we use them obliviously via the following lemma.
\begin{lemma}
\label{lem:sampling}
Let $\II\subseteq 2^I$ be a valid constraint,  $\bx \in P(\II)$ and $\delta>0$. Then, there is a polynomial time random algorithm which, given $\II$, $\bx$ and $\delta$, returns a random set $R\in \II$ for which the following hold.
\begin{enumerate}
	\item For any $i\in I$, $\Pr(i\in R) = (1-\delta)^2 \bx_i$.
	\item For any $\ba\in [0,1]^I$,  $\eps>0$  and $\zeta \geq (1-\delta)^2 \ba \cdot \bx$,
	$$\Pr\left(\sum_{i\in R} \ba_i \geq (1+\eps) \zeta \right)\leq \exp\left( -\frac{\zeta\cdot \delta\cdot \eps^2}{20}\right).$$
	\item Let $f:2^I\rightarrow \mathbb{R}_{\geq 0}$ be a submodular function such that $(\II,f)$ is  valid, $\eps>0$ and $\zeta \leq (1-\delta)^2 F(\bx)$, where $F$ is the multilinear extension of $f$. Also, let $f_{\max}= \max_{i\in I} f(\{i\})-f(\emptyset)$.
	 Then,
	$$\Pr\left(f(R) \leq (1-\eps)\zeta \right)\leq \exp\left(- \frac{\zeta\cdot  \delta\cdot \eps^2}{20 \cdot f_{\max}}\right).$$
\end{enumerate}
We say that the set $S$ is sampled by $\bx$, $\delta$ and $\II$.
\end{lemma}
Lemma \ref{lem:sampling} follows directly from \cite{CVZ10}, \cite{CVZ11}, the concentration bound of \cite{Vo10} (see Lemma \ref{lem:extension_cher}) and the Chernoff bounds of \cite{RKPS06} (see Lemma \ref{lem:chernoff}). %We note that the bounds in lemma can be tightened for specific cases, such that $\II=2^I$. However, we preferred to b


The rounding procedure is complemented with a procedure which finds a feasible assignment of the  sampled set $R$ for each  of the $d$-MKCs. Given a set $R\subseteq I'$, an MKC $(w,B,W)$, an $N$-leveled partition $(K_j)_{j=0}^{\ell}$, and $(\bx,\by^0,\ldots, \by^{\ell})\in P^e$, Algorithm \ref{alg:pack} ($\pack_{\delta}$, given in Section \ref{sec:packing_proof}), finds a feasible assignment $A$ for $(w,B,W)$. 
The next lemma states that with high probability $\bigcup_{b\in B} A(b) = R$.


\begin{lemma}
\label{lem:packing}
For any $\eps>0$ and $\delta\in\left(0,0.1\right)$, there is $N'_{\eps, \delta}$ such that, for any $N\geq N'_{\eps, \delta} $, there is $\gamma_{\eps,\delta, N}>0$ for which the following holds. 
For any  $\gamma \leq\gamma_{\eps,\delta,N}$, an MKC $(w,B,W)$ with an $N$-leveled partition $(K_j)_{j=0}^{\ell}$, and a valid constraint $\II$, let
$P^e$ be the extended $\gamma$-partition polytope of $(w,B,W)$ and $(K_j)_{j=0}^{\ell}$.  Given $(\bx, \by^0,\ldots, \by^{\ell})\in P^e$, let $R\subseteq 2^I$ be a random set sampled by $\bx$, $\delta$ and $\II$.
 Also, let $A$ be the output of Algorithm~\ref{alg:pack} for the above input. Then,
$$\Pr\left( \bigcup_{b\in B} A(b)\neq R\right)<\eps.$$
\end{lemma}
%	and $(\bx, \by^0,\ldots, \by^{\ell})\in P^e$, where $P^e$ is the extended $\gamma$-partition polytope of $(w,B,W)$ and $(K_j)_{j=0}^{\ell}$,  let $R\subseteq 2^I$ be a random set sampled by $\bx$, $\delta$ and $\II$.
%\yaron{need to address the technique/motivation of block association and bin-packing here.}

We give the proof of the lemma in Section~\ref{sec:packing_proof}.
Using the above techniques, we now 
formally present 
Algorithm \ref{alg:constant} and prove the next result. 
%Now that all techniques are presented, we can provide the algorithm, and prove the following lemma. 
%We consider the proof of the lemma, given in Section \ref{sec:packing}, and specifically the association mechanism used within the proof (Lemma \ref{lem:association}) to a significant contributions of this paper.\yaron{This paragraph shouldn't be here. Should be in results in some form.}




\begin{algorithm}
	\SetAlgoLined
	\SetKwInOut{Input}{Input}\SetKwInOut{Configuration}{Configuration}
	\DontPrintSemicolon
	
	\KwIn{A $d$-MKCP instance $\cT=\left(I,\left(w_t,B_t,W_t\right)_{t=1}^d,\II, f\right)$}
	\Configuration{Error parameters $\gamma, \delta>0$ and numbers $N>0$, $\xi>0$.}
	
	Initialize $T^*\leftarrow \emptyset$ and $D^*_t:B_t\rightarrow 2^I$ by $D^*_t(b)=\emptyset$ for every $1\leq t\leq d$ and $b\in B_t$. \;
	
	\ForAll{ $S\subseteq I$, $|S|\leq \xi$ and 
		feasible disjoint assignments $A_t$ of $S$  w.r.t. $(w_t, B_t, W_t)$ for $1\leq t\leq d$ \label{constant:loop}
	}{
		Let $\cT'=(I', \left(w_t, B_t, W'_t\right)_{t=1}^{d}, \II', g)$ be the residual instance of $\cT$, $S$, $(A_t)_{t=1}^{d}$ and $\xi$. \;
		
		Let $\tilde{B}_t, \tilde{W}_t$ be the $N$-leveled constraint of $B_t$, $W'_t$,  and let  $(K^t_j)_{j=0}^{\ell_t}$ be its $N$-leveled partition for $1\leq t\leq d$.
		\label{constant:leveling}
		\;
		
		
		Optimize $F(\bx)$ with $\bx \in P(\II') \cap \left(\bigcap_{t=1}^{d} P_t\right)$, where $P_t$ is the $\gamma$-partition polytope of $(w_t, \tilde{B}_t, \tilde{W_t})$ and $(K^t_j)_{j=0}^{\ell_t}$. \label{constant:opt} \;
		
		Let $R$  be a random set sampled by $\bx$, $\delta $ and $\II'$. 
		\label{constant:sampling}
		\;
		
		Let $\by^{t,0},\ldots, \by^{t,\ell_t}\in [0,1]^{I'}$ such that 
		$(\bx, \by^{t,0},\ldots, \by^{t,\ell_t})\in P_t^e$, where  $P_t^e$ is the extended $\gamma$-partition polytope of $(w_t, \tilde{B}_t,\tilde{W}_t)$ and the partition $(K^t_j)_{j=0}^{\ell_t}$ for $1\leq t\leq d$.\; 
		
		For $1\leq t \leq d$ set $A'_t =\pack_{\delta}\left(R, \left(w,\tilde{B}_t, \tilde{W}_t\right), \left(K^t_j\right)_{j=0}^{\ell_t},  (\bx,\by^{t,0},\ldots, \by^{t,\ell_t}) \right)$.\;
		
		\If{$\bigcup_{b\in \tilde{B}_t} A'_t(b)  = R$ for all $1\leq t\leq d$ and $g(R)\geq f(T^*)$}{
 			Set $T^*\leftarrow S\cup R$ .\;
 			
 			For $1\leq t \leq d$: set $D^*_t(b) \leftarrow A'_t(b) \cup A_t(b)$  for $b\in \tilde{B}_t$ and $D^*_t(b)\leftarrow A_t(b)$ for $b\in B_t\setminus \tilde{B}_t$.\;
		}
		
		
	}
	Return $T^*$ and $\left(D^*_t\right)_{t=1}^{d}$.\;
	\caption{$d$-MKCP} 
	\label{alg:constant}
\end{algorithm}

\begin{lemma}
	\label{lem:constant}
	For any $\eps>0$ and $d\in \mathbb{N}$ there are configuration parameters $\gamma$, $\delta$, $N$, and $\xi$ such that Algorithm \ref{alg:constant} returns a $(c-\eps)$-approximate solution for any $d$-MKCP, where $c=1$ if the value function is modular, $c=1-e^{-1}$ if the value function is monotone, and otherwise $c=0.385$.
\end{lemma}

\begin{proof}
Let $\eps>0$ and $d\in \mathbb{N}$. We select 
$N = \ceil{\max\left\{\frac{10\cdot d}{\eps^2} , N'_{\frac{\eps^2}{10\cdot d} , \eps^2}+1\right\}}$ and $\gamma = \gamma_{\frac{\eps^2}{10 \cdot d}, \eps^2,N}$  where $N'_{\frac{\eps^2}{10\cdot d} , \eps^2}$ and  $\gamma_{\frac{\eps^2}{10 \cdot d}, \eps^2,N}$ are defined in Lemma \ref{lem:packing}.
 %Also, select where $\gamma_{\frac{\eps^2}{10 \cdot d}, \eps^2,N}$ is defined by Lemma \ref{lem:packing}.
 Also, select $\delta = \eps^2$ and $\xi$ such that $\exp\left(-\frac{0.1\cdot (1-\eps^2)^4 \eps^6 }{20} \cdot \xi \right)\leq \frac{\eps^2}{10}$ and 
 $\frac{d\cdot N^2}{\gamma \cdot \xi}\leq \frac{\eps^2}{10}$. 
 
Let $\mathcal{T} = \left(I, \left( \mathcal{K}_t\right)_{t=1}^d, \II, f \right)$ be a $d$-MKCP instance. Also, let $S^*$ and $(A^*_t)_{t=1}^{d}$ be an optimal solution for $\mathcal{T}$, and $\OPT=f(S^*)$. W.l.o.g we assume that $A^*_t$ is a disjoint assignment for any $1\leq t\leq d$. 

By Lemma~\ref{lem:residual_generic}, there is $S\subseteq S^*$, $|S|\leq \xi$ such that $S^*\setminus S$ and $(A^*_t \setminus S)_{t=1}^{d}$ is a solution for $\mathcal{T}'$, the residual problem of $\mathcal{T}$, $S$, $(A^*_t\cap S)_{t=1}^{d}$ and $\xi$. From now on, we focus in the analysis on the iteration of the loop in Step \ref{constant:loop} in  which $S$ is the set defined above, and $A_t= A^*_t \cap S$ for any $1\leq t\leq d$. 

In Step~\ref{constant:leveling}, each of the MKCs are converted to an $N$-leveled constraint $\tilde{B}, \tilde{W}$. 
Recall that Lemma \ref{lem:structuring} bounds the decrease in the solution value due to such conversion.
Hence, by applying  the lemma iteratively, it follows that there is $\tilde{S}\subseteq S^*\setminus S$ such that $\tilde{S}$ is feasible for 
$(w_t,\tilde{B}_t, \tilde{W}_t)$ for any $1\leq t \leq d$ and 
 $g(\tilde{S})\geq \left( 1-\frac{d}{N}\right) g(S^* \setminus S)=\left( 1-\frac{d}{N}\right) \OPT$. Thus,
 it also holds that $\tilde{S}\in \II'$, as $S^*\setminus S\in \II$.
 
 For any $1\leq t \leq d$, let $D_t$ be a feasible assignment of $\tilde{S}$ for the MKC $(w_t,\tilde{B}_t, \tilde{W}_t)$.
  Denote by $V_t$ the set of $\gamma$-heavy items assigned to blocks with a single bin in $D_t$. That is,  $V_t = \bigcup_{j=0}^{\min\{\ell_t, N^2-1\}} \bigcup_{b\in K^t_j} D_t(b) \setminus L_{K^t_j, \gamma}$. 
  Since $|K^t_j|=1$ for any $0\leq j\leq \min\{N^2 -1 , \ell_t\}$, and $w(D_t(b))\leq W^*_{K^t_j}$ for $b\in K^t_{j}$, it follows that $|V_t| \leq \frac{N^2 }{\gamma}$. Let $V= \bigcup_{t=1}^d V_t$, thus $|V| \leq \frac{d\cdot N^2}{\gamma}$. Since $g$ is submodular, we have that
  $$g(\tilde{S}\setminus V)  \geq g(\tilde{S})  - |V| \cdot g_{\max} \geq
  \left( 1- \frac{d}{N} \right)\OPT -  \frac{d\cdot N^2}{\gamma} \cdot \frac{\OPT}{\xi} \geq (1-\eps^2)\OPT,$$
  where $g_{\max} = \max_{i\in I'} g(\{i\})-g(\emptyset) \leq\frac{f(S)}{\xi}\leq \frac{\OPT}{\xi}$.  For any $1\leq t\leq d$, $D_t\setminus V$ is an assignment of $\tilde{S}\setminus V$ w.r.t $(w_t, \tilde{B}_t,\tilde{W}_t)$ which satisfies the conditions of Lemma \ref{lem:gamma_soundness}, thus $\one_{\tilde{S}\setminus V} \in P_t$. 
  Furthermore, $\tilde{S} \setminus V\in \II'$ as $\tilde{S}\in \II'$. Hence, in Step \ref{constant:opt} the algorithm finds $\bx\in [0,1]^{I'}$ such that 
  $G(\bx)\geq c(1-\eps^2)\cdot g(\tilde{S}\setminus V) \geq c\cdot (1-\eps^2)^2 \OPT$, where $G$ is the multilinear extension of $g$ (if $g$ is modular this is achievable using the approximation scheme of Lemma \ref{lem:gamam_partitionpoly_fptas}).
  
  Recall that $R$ is the random set defined in Step \ref{constant:sampling}.
  Let $\Psi$ be the event in which $\bigcup_{b\in \tilde{B}_t} A'_t(b) = R$ for every $1\leq t \leq d$, and $g(R)\geq c\cdot (1-\eps^2)^5 \cdot \OPT$. 
  By Lemma \ref{lem:sampling}, it holds that 
  $$\Pr\left(g(R)< c\cdot (1-\eps^2)^5 \cdot \OPT \right)\leq \exp\left( -\frac{ (1-\eps^2)^4\cdot \eps^2 \cdot \eps^4\cdot c \cdot \OPT }{20 \cdot g_{\max}}\right)
  \leq 
  \exp\left( -\frac{ (1-\eps^2)^4 \cdot \eps^6\cdot c }{20}\xi\right)\leq \frac{\eps^2}{10}.$$
  Furthermore, by Lemma~\ref{lem:packing}, we have that 
  $\Pr\left( \bigcup_{b\in \tilde{B}_t} A'_t(b)\neq R\right) \leq \frac{\eps^2}{10d}$ for any $1\leq t\leq d$. Hence, by the union bound, $\Pr(\Psi)\geq (1-\eps^2)$. 
  
  Thus, subsequent to this specific iteration, it holds that 
  $$\E\left[ f(T^*)\right]\geq \Pr(\Psi)\E\left[g(R) ~|~\Psi\right] \geq (1-\eps^2)(1-\eps^2)^5\cdot c\cdot \OPT   \geq (c-\eps)\OPT,$$
  where the last inequality holds under the assumption that $\eps$ is sufficiently small, which can be assumed without loss of generality.
\end{proof}

Theorem \ref{thm:main} is essentially an immediate consequence of the above lemma.
\begin{proof}[Proof of Theorem \ref{thm:main}]
To complete the proof, given Lemma~\ref{lem:constant}, we only need to use the following observations. Algorithm \ref{alg:constant} always returns a feasible solution for the input instance. Furthermore, for any constant $\xi>0$, the algorithm is polynomial. 
\end{proof}



 






==> discussion.tex <==

In this paper we presented approximation algorithms for modular and submodular maximization with a constant number of multiple knapsack constraints and a possible additional constraint: matroid, matroid intersection, or matching. The approximation ratios achieved by our algorithms are optimal in the modular case and nearly optimal in the monotone submodular case. In the non-monotone submodular case our approximation ratio matches the best known ratio for non-monotone submodular optimization with a single knapsack constraint, which is a special case of our problem. We use as a key tool
the novel Fractional Grouping technique. The robustness of the technique is demonstrated by the broad range of algorithmic results. 

Our results for $d$-MCKP apply to instances in which the additional constraint, $\II$, and the objective function, $f$, form a valid pair. These restrictions
are derived from limitations of known concentration bounds for Randomized Swap Rounding \cite{CVZ10, CVZ11}, as 
formulated in Lemma~\ref{lem:sampling}.  
Specifically, Theorem II.2 in \cite{CVZ10} applies only to monotone submodular functions, while Theorem 1.1 in \cite{CVZ11} holds for modular functions.
 Deriving similar (possibly even weaker) bounds for a wider family of submodular functions may allow handling (in 
 Algorithm \ref{alg:constant}) a larger
 set of constraints $\II$ and functions $f$. For example,
extending Theorem II.2 in \cite{CVZ10} to non-monotone submodular functions will lead to an approximation algorithm for 
non-monotone submodular maximization with a multiple knapsack constraint and a matroid constraint.

We note that Fractional Grouping and Block Association can be applied also in conjunction with Contention Resolution Schemes (CR-schemes)~\cite{CVZ14}. This requires a mild adaptation of the  CR-schemes and may lead to approximation algorithms for problems that were not considered in this paper. One example is non-monotone submodular optimization with a multiple knapsack constraint and additional three matroid constraints. However, the  approximation ratios obtained by using CR-schemes were sub-optimal, and therefore not included in this paper.

Another desired goal is to improve 
the approximation ratio obtained for non-monotone $d$-MKCP. Here, an improvement in the ratio obtained for the multilinear optimization problem will lead to better approximation ratio for $d$-MKCP. 


Finally, we presented the first PTAS for the Multiple Choice Multiple Knapsack Problem, as a special case of modular  $d$-MKCP. The existence of an EPTAS for the problem remains
open. 




==> general.tex <==
In this section we provide a $(0.385-\eps)$-approximation for SMKP for any $\eps>0$. 
We start by extending the results of Section \ref{sec:block} for the case in which the set $B$ of bins has a partition $B=\bigcup_{j=1}^{\ell} K_j$ to blocks, in which the cardinality of  blocks, $|K_j|$,  is either large or is one. We obtain the following result for such instances.
\begin{lemma}
\label{lem:block_partition}
For any $\delta>0$ there is $N_{\delta}>0$ such that Algorithm \ref{alg:partition} satisfies the following.
Given  an SMKP  instance and a partition of the set $B$ of bins into blocks  $B=\bigcup_{j=1}^{\ell}K_j$  such that $|K_j|\geq N_{\delta}$ or $|K_j|=1$, Algorithm \ref{alg:partition} returns a feasible assignment $A$ such that 
$f\left( \bigcup_{b\in B} A(b)\right) \geq (c-\delta)\OPT- 2\cdot s\cdot  f_{\max}$ 
where $f_{\max}= \max_{i\in I} f(\{i\})$, 
$c=1-e^{-1}$ if $f$ is monotone and $c=0.385$ if $f$ is non-monotone,
 and $s=\left|\left\{1\leq j \leq \ell ~|~|K_j|=1\right\}\right|$. 
\end{lemma}


The result in Lemma \ref{lem:block_partition} can be combined with known enumeration and structuring techniques to obtains a
$(0.385-\eps)$-approximation for general SMKP instances.
The enumeration reduces the input instance to a new instance  where  $ f_{\max}$ is bounded. The structuring (see \cite{FKNRS20}) ensures the existence of a partition of the bins to blocks such that $s$ is bounded.
 
%By combining Lemma \ref{lem:block_partition} with known enumeration and structuring techniques (i.e., reducing the number of blocks in the instance) we obtain a $(0.385-\eps)$-approximation for general SMKP instances.


\subsection{Multiple Blocks}

Let $(w,B,W)$ be an MKS and let $\left(K_j\right)_{j=1}^{\ell}$ be a partition of $B$ to blocks. That is, $K_j$ is a block for every $1\leq j \leq \ell$, the sets $K_1,\ldots, K_{\ell} $ are disjoint and $B= \bigcup_{j=1}^{\ell} K_j$. We assume $(w,B,W)$ and the partition $\left( K_j\right)_{j=1}^{\ell}$ are fixed through the section.

\begin{defn}
\label{def:extended_partition}
The  extended partition polytope of $(w,B,W)$ and $\left(K_j\right)_{j=1}^{\ell}$ is
\begin{equation}
\label{eq:ex_partition}
P^e= \left\{ (\bx, \by^1, \ldots, \by^\ell)~\middle|~ \bx \in [0,1]^I,~ \forall  1\leq j \leq \ell: \by^{j}\in P_{K_j},~ \sum_{j=1}^{\ell} \by^j = \bx\right\}.
\end{equation}
where $P_{K_j}$ is the block polytope of $K_j$ (see Definition \ref{def:block_polytope}).  
\end{defn}
\begin{defn}
The   partition polytope of $(w,B,W)$ and $\left(K_j\right)_{j=1}^{\ell}$ is
\begin{equation}
\label{eq:partition}
P= \left\{ \bx  \in [0,1]^I~\middle|~ \exists \by^1,\ldots \by^{\ell} \in [0,1]^I \text{ s.t. } (\bx, \by^1, \ldots, \by^\ell) \in P^e~\right\}.
\end{equation}
where $P^e$ is the extended partition  polytope of $(w,B,W)$ and $\left(K_j\right)_{j=1}^{\ell}$.
\end{defn}

As in the case of the block polytope, though 
 $\max_{\bx\in P} \bc \cdot \bx$ cannot be solved exactly in polynomial time, it can  be approximated, as stated in the following lemma.
\begin{lemma}
	\label{lem:_partitionpoly_fptas}
	%\comment{
	There is a fully polynomial approximation scheme for the problem of finding $\bx \in P$ such that $\bx \cdot \by$ is maximal, given an $MKS$ $(w,B,W)$, a partition $\left(K_j\right)_{j=1}^{\ell}$ of the bins   $B$ to blocks and a vector $\bc\in \mathbb{R}^I$, where $P$ is the partition polytope of $\left(K_j\right)_{j=1}^{\ell}$ . 
	%}
	%$P_K$ is approximable. 
\end{lemma}
A detailed proof of the lemma is given in the Appendix (\ariel{TBD}).

As in the case of the block polytope, the partition polytope is sound for the problem.
\begin{lemma}
	\label{lem:part_soundness}
	Let $A$ be a feasible assignment for $(w,B,W)$ and $S=\bigcup_{b\in B} A(b)$. Then $\one_S \in P_K$. 
\end{lemma}
Let $(\bx , \by^1,\ldots, \by^{\ell})\in P_K$ and $\aeps\in \left(0,\frac{1}{2}\right]$. %Denote $\supp(\bx)=\{i\in I ~|~\bx_i>0\}$. 
 Our  overall objective is to convert $\bx$ into a feasible assignment. The first step in the process is to allocate the items to blocks. Afterwards, a pipage rounding procedure similar to the one of Algorithm \ref{alg:uniform} is applied to each block. 

\comment{
We use an abstract notion of constraints. For a set $S$, $\bc\in \mathbb{R}_{\geq 0}^S$  and $\beta \in \mathbb{R}_{\geq 0}$, we say $\bgam\in [0,1]^{S}$ {\em satisfies $(S,\bc, \beta)$} if $\sum_{i\in S} \bc_i \cdot \bgam_i \leq \beta$. We say $\bgam\in [0,1]^{S}$ {\em semi-satisfies $(S,\bc, \beta)$} if it satisfies $(S,\bc, \beta)$, or there is $i^*\in S$ such that  $\sum_{i\in S\setminus\{i^*\}} \bc_i \cdot \bgam_i \leq \beta$.  We refer to $(S,\bc,\beta)$ as a {\em constraint}. The following lemma is central for the association of items to blocks.
}




The result of Lemma \ref{lem:association} is a key for Algorithm \ref{alg:partition}. Similarly to the case of uniform bins (Algorithm \ref{alg:uniform}), the algorithm first obtains a solution $\bx\in P$ for the multilinear extension such that the value of $F(\bx)$ is high.
The association of $(I_j)_{j=1}^{\ell}$ determines that the items in $I_j$ will be packed into the bins of $K_j$. Using this association,  Pipage rounding can be used to round the entries of $I_j$ in  $\bx$. For blocks $j\in M$ we use $\BlockPipage$, which was already used in the uniform case. For blocks $K_j=\{b\}$, the rounding only concerns the overall weight of items assigned to $b$, and a single item may be removed from the assignment after the rounding to ensure feasibility.

\begin{algorithm}
	\SetAlgoLined
	\SetKwInOut{Input}{Input}\SetKwInOut{Configuration}{Configuration}
	\DontPrintSemicolon
	
	\Input{An MKS $(w,B,W)$ over $I$. A partition $(K_j)_{j=1}^{\ell}$ of the bins to blocks. A value $N$ such that $|K_j|=1$ or $|K_j|\geq N$ for every $1\leq j \leq N$. A submodular function $f:2^I\rightarrow \mathbb{R}_{\geq 0}$. An error parameter $\delta>0$. }
	
	\label{uniform:opt}
	Find an approximate solution $(\bx,\by^1,\ldots, \by^{\ell}) \in P^e$ for $\max_{(\bx^0,\by^1,\ldots, \by^{\ell}) \in P^e} F(\bx)$, where $P^e$ is the the extended partition polytope of $(K_j)_{j=1}^{\ell}$. \;
	
	Select $\aeps = \min\left\{
	\frac{\eps}{4},  \frac{1}{2}\right\}
	$ .\;
	
	Update $(\bx,\by^1,\ldots, \by^{\ell}) \leftarrow (1-\eps) \cdot (\bx^0,\by^1,\ldots, \by^{\ell})$. \label{partition:scale}\;
	
	%Let $G^j_1, \dots, G^j_{\tau^j}$ be the $\aeps$-partition of $\by^j$ with respect to the block $K_j$. \;
	Let $(I_j)_{j=1}^{\ell}$ be the association of $(\bx,\by^1,\ldots, \by^{\ell})$.\;
	
	Initialize $A:B\rightarrow 2^I$ by $A(b)=\emptyset $ for every $b\in B$. 

	\For{$j\in M$}{
		%\For{$k=1,2,\ldots, \tau$}{
		%	$\bx  \leftarrow \pipage\left(\bx,f,G_k \cap I_j , \bar{1}\right)$. \;
		%}
		%$\bx = \pipage\left(\bx,f,L_{K_j,\aeps} \cap I_j, \left(w(i) \right)_{i\in L_{K_j, \aeps}\cap I_j}\right)$.\;
		
		%Let $S_j=\{i\in I_j ~|~ \bx_i = 1\}$\;
		
		%Pack the items in $S_j$ into bins of capacity $W^*_K$ using the algorithm of \cite{KK82}. Let $D_1,\ldots, D_{\eta_j}$ be the output of the algorithm.

		%\;
		%Let $K_j=\{b_1,\ldots, b_{|K_j|}\}$. \;
		%Define $A(b_r)= D_r$ for $1\leq r \leq \min\{|K_j|,\eta_j\}$ and $A(b_r)= \emptyset$ for $\min\{|K_j|,\eta_j\}< b\leq |K_j|$. \;
		$\bx, A_j\leftarrow \BlockPipage(\bx, K_j, I_j,\by^j, \aeps)$ ($\BlockPipage$ is defined in Algorithm \ref{alg:block_pipage}).
		\label{partition:block_pipage}
		\;
		Set $A(b)= A_b(b)$ for every $b\in K_j$. 
	}
	\For{$j\in \{1,\ldots, \ell \}\setminus M$} {

		Let $i^*_j\in I_j$ such that $\sum_{i\in I_j\setminus \{i^*_j\}} w(i)\cdot \bx_i \leq \sum_{i\in I } w(i) \cdot \by^j_i$.
				\label{partition:find_i_star}
				\;
		
		$\bx  \leftarrow \pipage\left(\bx,f, I_j \setminus\{i^*_j\},\left(w(i) \right)_{i\in I_j\setminus \{i^*_j\}} \right)$. \;
		
		%Let $S_j = \{i\in I_j\setminus \{i^*_j\} ~|~\bx_i=1 \}$ \;
		
		Find $i'_j\in I$ such that $w(S_j) \leq W^*_{K_j}$ where $S_j= \{i\in I_j~|~\bx_i=1\}\setminus\{i'_j,i^*_j\}$.\label{partition:find_i_prime}\;
		Let $K_j=\{b\}$, and set
		$A(b)=S_j$. \label{partition:singleton} \; 
	}
	Return $A$\;
	\caption{Submodular Multiple Knapsack with Bin Partition} 
	\label{alg:partition}
\end{algorithm}
\begin{proof}[Proof of Lemma \ref{lem:block_partition}]
	
Let $\delta>0$, and let $N_{\delta}>0$ such that for any $N'>N_{\delta}$ it holds that   $-\aeps\cdot N'+4 \cdot 4^{ \aeps^{-2}}+ 10+\rho \log^2 N'\leq 0$ where $\aeps = \min \left\{ \frac{\delta}{4}, \frac{1}{2}\right\}$ and $\rho$ is a constant such that the algorithm of \cite{KK82} returns a bin packing using $\OPT+\rho \log^2\OPT$ bins for every bin packing instance. 
\ariel{it may be nice to find the numbers in order to be able to provide the running time dependency of the algorithm in $\delta$, also, revisit the number after section 1 is updated.}

Consider the the execution of Algorithm \ref{alg:partition} with $N_{\delta}$ and $\delta$. 
We first observe the algorithm always finds an item in Step \ref{partition:find_i_star}
due to Lemma \ref{lem:association}. Futheremore, 
following Lemma \ref{lem:pipage}, on the execution of Step \ref{partition:find_i_prime} an $i'_j$ satisfying the condition exists since $\sum_{i\in I }\by^j_i \cdot  w(i) \leq W^*_K$  as $\by^j\in P_{K_j}$. We note that at any point of the algorithm's execution the assignment $A$ is feasible, and therefore the algorithm returns a feasible assignment.

Let $\OPT$ the optimal value of the SMKP instance. 
It follows that $F(\bx^0)\geq c \cdot  \OPT$. As
the second derivatives of $F$ are negative, following the execution of  Step \ref{partition:scale} it holds that 
$F(\bx)\geq (1-\delta)\cdot  c\cdot \OPT\geq (c-\delta)\cdot  \OPT$. 
By the properties of Pipage rounding (Lemma \ref{lem:pipage}), it follows that upon the termination of the
algorithm it also holds that $F(\bx ) \geq (c-\delta)\cdot  \OPT$. 

Let $\{i\in I~|~\bx_i=1\}\subseteq T\subseteq \supp(\bx)$ such that $f(T)$ is maximal. By the definition of the multilinear extension it holds that 
$f(T)\geq F(\bx) \geq (c-\delta)\cdot  \OPT$. 
For $j\in M$ let $S_j$ and $\eta_j$ be the values of the  $S$ and $\eta$ on the execution of Algorithm \ref{alg:block_pipage} when invoked for $j$ in Step \ref{partition:block_pipage}. 
 By the end of the algorithm's execution it holds that $ \supp(\bx)\setminus \left( \bigcup_{j=1}^{\ell} S_j\right)
 \subseteq \{i^*_j,i'_j~|~ 1\leq j\leq k,~j\notin M\}
 $, and furthermore $\bigcup_{j=1}^{\ell} S_j\subseteq T$.
 %,  it follows that $|T\setminus| \leq |\{i^*_j, i'~|~ 1\leq j\leq k,~j\notin M\}| =s$ (the value of $s$ is defined in statement of the lemma, and equals to $\ell - |M|$). 
  Hence,
 $$f(T)= f\left(\bigcup_{j=1}^{\ell} S_j\right) +  f_{\bigcup_{j=1}^{\ell} S_j} \left(T\setminus \bigcup_{j=1}^{\ell} S_j\ \right)\leq f\left(\bigcup_{j=1}^{\ell} S_j\right)   +2\cdot s\cdot f_{\max}.$$
 Recall $s$ and $f_{\max}$ were defined in statement of the lemma.
 Therefore we have $f\left(
 \bigcup_{j=1}^{\ell} S_j
 \right)   \geq f(T) - 2\cdot s \cdot f_{\max}\geq (c-\delta)\OPT -2\cdot s \cdot f_{\max}$. 
 
To complete  the proof it suffices to show that $ \bigcup_{b\in B} A(b)= \bigcup_{j=1}^{\ell} S_j$. For any $k\in M$, by Lemmas \ref{lem:association} and \ref{lem:pipage} it holds that for any $1\leq k\leq \tau_j$ we have that $|S_j\cap G^j_k|\leq \aeps|B| + 3$, and similarly
$w(S_j \cap L_{K_j,\aeps}\setminus {i'_j})\leq \sum_{i\in L_{K_j,\aeps} } \by^j_i \cdot w(i) +2 \aeps W^*_{K_j}$. Hence, following Lemma \ref{lem:second_creteria} it holds that 
$S_j$ can be packed into $(1-\aeps) |K_j| +3\cdot  4^{\aeps^{-2}} + 10+\leq |K_j|$ bins of capacity $W^*_{K_j}$. Thus, it holds that $\eta_j \leq   
(1-\aeps) |K_j| +3\cdot  4^{\aeps^{-2}} + 10+\rho^2 \log |K_j|\leq |K_j|$, and we have that $\bigcup_{b\in K_j } A(b)=S_j$. Also, for $1\leq j \leq \ell$, $j\notin M$ it holds that $\sum_{b\in K_j} A(b)=S_j$ as a consequence of Step \ref{partition:singleton}. Overall, it holds that 
$ \bigcup_{b\in B} A(b)= \bigcup_{j=1}^{\ell} S_j$ which completes the proof.
 
 
\end{proof}

\subsection{The General Case}

%We use enumeration along with structuring in order to obtain an approximation algorithm for generic instances. Enumeration, along with the concept of residual instances, is commonly used for submodular and modular optimization with knapsack constraint \cite{KST13, CVZ10, khuller1999budgeted, FKNRS20}. Structuring is often used for multiple knapsack problem \cite{FKNRS20}. 
We first describe the enumeration and structuring techniques used for deriving approximation algorithms for generic SMKP instaces.

Given an SMKP $\cT=(I,(w,B,W), f)$, 
let $A$ be a solution for $\cT$,
and let $\xi\in \mathbb{N}$. We define the {\em residual instance of $\cT$,  $A$ and $\xi$} as the SMKP instance 
$\cT'=(I',(w,B,W'), g)$, where
\begin{enumerate}
	\item
	$I'=\left\{ i\in I\setminus S ~\middle|~ f(\{i\}\cup S )-f(S)\leq \frac{f(S)}{\xi}\right\}$ , where $S=\bigcup_{b\in B} A(b)$.
	\item The function 
	$g:2^{I'}\rightarrow \mathbb{R}_{\geq 0}$ is defined by $g(T)=f(S\cup T)$ (with $S=\bigcup_{b\in B} A(b)$ as before).
	\item $W'(b)= W(b) - w(A(b))$ for all $b\in B$.
\end{enumerate}

We note that the function $g$ is submodular and non-negative. Furthermore, $g$ is monotone if $f$ is monotone (see Lemma \ref{lem:submodular_cup}). 
It can be easily verified that, if $A':B\rightarrow 2^{I'}$ is a solution for the residual 
instance $\mathcal{T}'$, then $A\cup A'$  is a solution for the original instance $\mathcal{T}$. Furthermore, by definition, $f\left(\bigcup_{b\in B} A(b)\cup A'(b)\right)=g\left(\bigcup_{b\in B} A'(b)\right)$.  \ariel{verify operations over assignments are defined.}

Our algorithm uses enumeration in order to find the assignment $A^*\cap S$ whose existence  is guaranteed by the following lemma.\footnote{Given an assignment $A:B\rightarrow 2^I$ and a set $S\subseteq I$, we define $A\cap S$ to be the assignment $D:B\rightarrow 2^I$ such that $D(b)=A(b)\cap S$ for every $b\in B$. }
\begin{lemma}
	\label{lem:residual}
	Let $\xi\in \mathbb{N}$, $\mathcal{T}$ be an SMKP instance, and $A^* $be  a (possibly optimal) solution for $\mathcal{T}$. Then there is 
	$S\subseteq \bigcup_{b\in B} A^*(b)$, $|S|\leq \xi$  such that $(A^*\setminus S)$ is a solution for the residual instance of 
	$\mathcal{T}$,  $A^*\cap S$ and $\xi$.
\end{lemma}
\ariel{Decide what to do regarding the proof.}

We use the structuring technique of  \cite{FKNRS20} to reduce a given MKS into a new MKS with bins satisfying the following property. 
\begin{defn}
	For any $N\in \mathbb{N}$, a set of bins $B$ and capacities $W:B\rightarrow \mathbb{R}_{\geq 0}$,  we say that a partition $(K_j)_{j=1}^\ell$ of $B$
	is {\em $N$-leveled} if for all $0\leq j \leq \ell$ it holds that $K_j$ is a block, and  $|K_j|= N^{\floor{\frac{j}{N^2}}}$. 
\end{defn}
 This reduction, as guaranteed by the next lemma, preserves the values of solutions for the original MKS, up to a small error. 


\begin{lemma}
	\label{lem:structuring}
	For any $N$, set of bins $B$ and capacities $W:B\rightarrow \mathbb{R}_{\geq 0}$, there is $\tilde{B}\subseteq B$,  capacities $\tilde{W}:\tilde{B}\rightarrow \mathbb{R}_{\geq 0}$,
	and an $N$-leveled partition  $(\tilde{K}_j)_{j=0}^\ell$ of $\tilde{B}$,
	such that
	\begin{enumerate}
		\item $\tilde{B}$, $\tilde{W}$ and $(\tilde{K}_j)_{j=0}^\ell$ can be computed in polynomial time.
		\item
		The bin capacities satisfy $\tilde{W}(b) \leq W(b)$, for every $b\in \tilde{B}$.
		\item
		\label{structuring_prop2}
		For any set of items $I$, weight function  $w:I\rightarrow \mathbb{R}_{\geq 0}$, a subset $S\subseteq I$ feasible for the MKS $(w,B,W)$ over $I$, and a submodular function $f:2^I \rightarrow \mathbb{R}_{\geq 0}$, there is  $\tilde{S}\subseteq S$ feasible for the MKS $(w,\tilde{B},\tilde{W})$ such that $f(\tilde{S}) \geq \left(1- \frac{1}{N}\right) f(S)$.
	\end{enumerate}
	We refer to $\tilde{B}$ and $\tilde{W}$ as the $N$-leveled instance of $B$ and $W$. 
\end{lemma}

The proof of the lemma is a minor extension over the results of \cite{FKNRS20}. We provide a full proof in Appendix \ref{sec:structuring} for completeness. \ariel{mention that a weaker structuring can be used? I am not sure it will be clear}

\begin{algorithm}
	\SetAlgoLined
	\SetKwInOut{Input}{Input}\SetKwInOut{Configuration}{Configuration}
	\DontPrintSemicolon
	
	\Input{An SMKP instance $\cT=(I,(w,B,W),f)$}
	\Configuration{Error parameter $\delta>0$ and numbers $N>0$, $\xi>0$.}
	
	Initialize $D:B\rightarrow 2^I$ by $D(b)=\emptyset$ for every $b\in B$. \;
	
	\ForAll{feasible disjoint assignment $A$  w.r.t. $(w, B, W)$ such that $\left| \bigcup_{b\in B} A(b)\right|\leq \xi$ \label{generic:loop}
	}{
		Let $\cT'=(I', (w, B, W'), g)$ be the residual instance of $\cT$, $A$ and $\xi$. \;
		
		Let $\tilde{B}, \tilde{W}$ be the $N$-leveled instance of $B$, $W'$,  and let  $(K_j)_{j=0}^{\ell}$ its $N$-leveled partition.\;
		
		Let $A'$ be the assignment returned by Algorithm \ref{alg:partition} with $\tilde{\cT}=(I',(w,\tilde{B},\tilde{W}), f)$, the partition $(K_j)_{j=0}^{\ell}$ and the parameters $\delta$,  $N$.
		
		If $f\left(\bigcup_{b\in B} A(b)\cup A(b')\right)\geq 
		f\left(\bigcup_{b\in B} D(b)\right)$ update $D\leftarrow A' \cup A$. 
	}
	Return $D$\;
	\caption{Submodular Multiple Knapsack} 
	\label{alg:generic}
\end{algorithm}

\begin{lemma}
	For any $\eps>0$ there are parameters $\delta, N, \xi$ such that Algorithm \ref{alg:generic} is a $0.385-\eps$-approximation algorithm for the Submodular Multiple Knapsack Problem.
\end{lemma}
\begin{proof}
Let $\eps>0$, and define $\delta= \frac{\eps}{4}$,  $N=\max\left\{\frac{4}{\eps}, N_{\delta} \right\}$ ($N_{\delta}$ is defined in Lemma \ref{lem:block_partition}), and finally set $\xi = \frac{6\cdot N^2}{\eps}$. 

Consider the execution of Algorithm \ref{alg:generic} with the above parameters and SMKP instance $\cT=(I,(w,B,W),f)$. Let $A^*$ be an optimal solution for the instance, and let $\OPT=f\left(\bigcup_{b\in B } A^*(b)\right)$ be its value. By Lemma \ref{lem:residual} there is $S\subseteq \bigcup _{b\in B} A^*(b)$, $|S|\leq \xi$ such that $A^*\setminus S$ is a solution for the residual instance of $\cT$, $A^*\cap S$ and $\xi$. 

Our analysis focuses on the iteration of  the loop in Step \ref{generic:loop} in which $A=A^*\cap S$. Thus, $A^*\setminus S$ is a solution for $\cT'$, therefore the value of the optimal solution of $\cT'$ is at least $g=\left(\bigcup_{b\in B } A^*(b)\setminus S\right)=f\left(\bigcup_{b\in B } A^*(b)\right)=\OPT$. Hence, by Lemma \ref{lem:structuring} it holds that the value of the optimal solution of $\tilde{\cT}$ is at least 
$\left(1-\frac{1}{N}\right) \OPT\geq\left(1-\frac{\eps}{4}\right)\OPT$. 
Let $g_{\max}= \max_{i\in I'} g(\{i\})$, following the definition of a residual instance it holds that $g_{\max}\leq \frac{f(S)}{\xi}\leq \frac{\OPT}{\xi}$ (note that $A^*\cap S$ is a feasible solution). By Lemma \ref{lem:block_partition} it holds that 
\begin{equation*}
\begin{aligned}
f&\left(\bigcup_{b\in B} A(b)\cup A'(b)\right)
=g\left(\bigcup_{b\in \tilde{B}} A'(b) )\right) \geq \left(0.385 - \frac{\eps}{4}\right)\left(1-\frac{\eps}{4}\right)\OPT -2\cdot N^2 \cdot g_{\max }\\
&\geq \left(0.385-\frac{\eps}{2}\right)\OPT - \frac{2\cdot N^2}{\xi} \OPT \geq \left( 0.385-\eps\right)\OPT
\end{aligned}
\end{equation*} 
 Hence, following this  iteration it holds that $f\left( \bigcup_{b\in B} D(b)\right)\geq (c-\eps) \OPT$.
 
Furthermore, for fixed $\xi$ the running time of the algorithm is polynomial, thus it is a $(0.385-\eps)$-approximation for SMKP.
\end{proof}






==> nonmon.tex <==

In this section we provide an approximation algorithm for non-monotone $d$-MKCP with no additional constraint. As in Section~\ref{sec:algorithm}, the reduction to restricted instances (Lemma~\ref{lem:restricted}) and  the $\gamma$-instance polytope  (Definition~\ref{def:poly_instance}) are utilized. However, we do not use submodular concentration bounds (see Lemma~\ref{lem:sampling}), as in Section~\ref{sec:algorithm}, since those depend on the maximal absolute marginal value of an item $\max_{i\in I} \left|f(\{i\})-f(\emptyset)\right|$. 
In the monotone and modular cases the reduction to restricted instances ensures the marginal absolute value of  an item is bounded. However, this reduction does provide a similar bound in the non-monotone case. Hence, 
we resort to  {\em contention resolution schemes}~\cite{CVZ14}  to obtain the approximation guarantee. 

To simplify the presentation, we provide a limited definition of contention resolution schemes which suffices to our setting. We refer the reader to~\cite{CVZ14} for a more  general definition. 
\begin{defn}
\label{def:contention}
Let $\cT=\left(I,\left(\mathcal{K}_t\right)_{t=1}^d,\II, f\right)$  be a $d$-MKCP instance and $P$ its $\gamma$-instance polytope for some $\gamma>0$. A monotone $(b,c)$-balanced  contention resolution scheme, where $b,c\in [0,1]$,  is a function $\pi: b\cdot P \times 2^I \rightarrow 2^I$ satisfying the following properties:
\begin{enumerate}
	\item For all  $\bx \in b\cdot P$ and $S\subseteq I$ it holds that  $\one_Q \in P$ where $Q=\pi(\bx, S)$.
	\item For any $\bx \in b \cdot P$  and $i\in \supp(\bx)$ it holds that $\Pr\left( i\in \pi (\bx, R)~\middle|~i\in R\right)\geq c$, where $R\sim \bx$. 
	\item For any $\bx\in b\cdot P$,  $S_1\subseteq S_2\subset I$ and $i\in S_1$ such that $i\in \pi(\bx, S_2)$, it also holds that $i\in \pi(\bx, S_1)$. 
\end{enumerate}
\end{defn}
For simplicity, we say $\pi$ is a $(b,c)$-scheme if it is a $(b,c)$-balanced monotone contention resolution scheme. In~\cite{CVZ14} the authors also define a {\em pruning} function $\eta_f$ for every  submodular function $f:2^I\rightarrow \mathbb{R}$.
We refer the reader to~\cite{CVZ14} for the formal definition of the function.  It holds that $\eta_f(S)\subseteq S$ and $f(\eta_f(S))\geq f(\emptyset)$ for every $S\subseteq I$. Furthermore, $\eta_f(S)$ can be evaluated using $O(|S|)$ oracle queries of~$f$. 
We utilize contention resolution schemes through the following lemma.
\begin{lemma}[Theorem 1.3 of \cite{CVZ14}]
Let $\cT=\left(I,\left(\mathcal{K}_t\right)_{t=1}^d,\II, f\right)$  be a $d$-MKCP instance with a partition of the MKCs to blocks, $P$ its $\gamma$-instance polytope for some $\gamma>0$, and $\pi$ be a  $(b,c)$-scheme.
Then for any $\bx \in b\cdot P$ it holds that 
$$E\left[ f\left(\eta_f( \pi(\bx, R) ) \right)\right]\geq c\cdot F(\bx),$$ 
where $R\sim \bx$, $F$ is the multilinear extension of $f$, and $\eta_f$ is the pruning function of $f$.
\end{lemma}

In the following we will generate a $(1-\delta, 1-\delta)$-scheme for non-monotone  $(N,\xi)$-restricted valid $d$-MCKP instances with no additional constraints. \ariel{update the ratio} Towards this end we use the following technical definition.

\begin{defn}
\label{def:complaint}
Fix $\delta>0$, and $\gamma>0$. 
Let $\cT=\left(I,\left(w_t, B_t,W_t\right)_{t=1}^d,\II, f\right)$  be a $d$-MKCP instance with a partition $(K^t_j)_{j=0}^{\ell_t}$ of $B_t$ to blocks for $1\leq t\leq d$, $P$ be its $\gamma$-instance polytope and $\bx\in P$. 
Let $\by^{t,0},\ldots, \by^{t,\ell_t}\in [0,1]^I$ such that $(\bx,\by^{t,0},\ldots, \by^{t,\ell_t})\in P^e_t$ for $1\leq t\leq d$, where $P^e_t$ is the $\gamma$-partition polytope of $(w_t,B_t,W_t)$ and $(K^t_j)_{j=0}^{\ell_t}$.
We say that $S\subseteq \supp(\bx)$ is {\em compliant} if the following holds:
\begin{enumerate}
	\item For any $1\leq t\leq d$ and $0\leq j \leq \ell_t$  such that   $|K^t_j|=1$ it holds that 
	$w_t(S\cap I^t_j) \leq W^*_{K^t_k}$.
	\item 
	For any $1\leq t\leq d$ and $1\leq j\leq \ell_t$ such that $|K^t_j|>1$ it holds that:
	\begin{enumerate}
		\item $w(S\cap I^t_j \cap  L_{K^t_j, \aeps} ) \leq \sum_{i\in L_{K^t_j,\aeps} } (1-\delta) \cdot \by^{t,j}_i \cdot w_t(i)+ \frac{\aeps}{4}\cdot W^*_{K^t_j} \cdot |K^t_j|$. 
		\item
		$|S\cap G^{t,j}_k \cap I^t_j| \leq \aeps \cdot |K^t_k|$ for any $1\leq k\leq \tau_{t,j}$. 
	\end{enumerate}
\end{enumerate}

Where,
\begin{itemize}
	\item $\aeps = \frac{\delta}{4}$. 
	\item 
 $G^{t,j}_{1},\ldots, G^{t,j}_{\tau_{t,j}}$ is  the $\aeps$-grouping of $(1-\delta)\cdot \by^{t,j}$ for any $1\leq t\leq d$ and $0\leq j\leq \ell_t$ such that $|K^t_j|>1$. 
 \item $(I^t_j)_{j=0}^{\ell_t}$ is the block association of $(1-\delta) (\bx,\by^{t,0},\ldots, \by^{t,\ell_t})$ for $1\leq t\leq d$.  
\end{itemize}
\end{defn} 
\ariel{yes, the definition is terrible. I am not sure how ot make it more pleasant at the moment.}



\begin{algorithm}
	\SetAlgoLined
	\SetKwInOut{Input}{Input}\SetKwInOut{Configuration}{Configuration}
	\DontPrintSemicolon
	
	\KwIn{A modular or monotone  $(N,\xi)$-restricted valid $d$-MKCP instance $\mathcal{R}$ defined by  $\left(I,\left(w_t,B_t,W_t\right)_{t=1}^d,\II, f\right)$ and $(K^t_j)_{j=0}^{\ell_t}$ the $N$-leveled partition of $B_t$ for $1\leq t\leq d$.}
	\Configuration{$\gamma>0$, $\delta>0$, $N\in\mathbb{N}$, $\xi\in \mathbb{N}$,}
	
	
	
	Optimize $F(\bx)$ with $\bx \in P$, where $P$ is 
	$\gamma$-instance polytope of the $\mathcal{R}$, and $F$ is the multilinear extension of $f$. \label{restricted:opt} \;
	
	Let $R$  be a random set sampled by $\bx$, $\delta $ and $\II'$. 
	\label{restricted:sampling}
	\;
	
	Let $\by^{t,0},\ldots, \by^{t,\ell_t}\in [0,1]^{I}$ such that 
	$(\bx, \by^{t,0},\ldots, \by^{t,\ell_t})\in P_t^e$, where  $P_t^e$ is the extended $\gamma$-partition polytope of $(w_t, B_t,W_t)$ and the partition $(K^t_j)_{j=0}^{\ell_t}$ for $1\leq t\leq d$.
	\label{restricted:defs}\;
	
	Find the association $(I^t_j)_{j=0}^{\ell_t}$ of $(1-\delta)(\bx, \by^{t,0},\ldots, \by^{t,\ell_t})$ and $\aeps=\frac{\delta}{4}$ for $1\leq t \leq d$. \label{restricted:association}\;
	
	Pack the items of $R\cap I_j^t$ into the bin of $K^t_j$ using an algorithm for bin packing if $|K^t_j|>1$, or simple assign $R\cap I_j^t$ to  $K^t_j$ otherwise . \label{restricted:packing} \;
	
	Return $R$ and the resulting assignment if the above step succeeded. Otherwise return an empty set and an empty packing. \label{restricted:return}
	\;
	
	\caption{$(N,\xi)$-restricted $d$-MKCP} 
	\label{alg:restricted}
\end{algorithm}



==> packing.tex <==


In this section we present the packing  procedure $\pack$ used by Algorithm \ref{alg:constant}. 
Given a set $R\subseteq I$, the procedure finds (with high probability) an assignment $A$ of $R$. To do so, $\pack$ 
associates each item in $R$ with a block $K_j$, and then
attempts to pack the items associated with $K_j$ into  its bins using a Bin Packing algorithm (similar to Algorithm \ref{alg:uniform}).
%
%ga partition $(S_j)_{j=0}^{\ell}$ of $S$ and attempts to pack the items of $S_j$ into the bins of the block $K_j$ by a Bin Packing algorithm, similarly to Algorithm \ref{alg:uniform}.
%The heart of the procedure is the generation of the partition $(S_j)_{j=0}^{\ell}$. In fact, the algorithm generates a partition $I_0,\ldots, I_{\ell}$ of $\{i\in I ~|~ \bx_i >0\}=\supp(\bx)$ which is independent of $S$, and then defines $S_j=S\cap I_j$. 
%
The Block Association procedure is presented in Section \ref{sec:association}.
%
%the method by which the partition $I_0,\ldots, I_{\ell}$, referred as {\em association} is found.
 Subsequently, in Section \ref{sec:packing_proof} we describe the $\pack$ procedure and give the proof of Lemma \ref{lem:packing}.



\subsection{Proof of Lemma \ref{lem:packing}}
\label{sec:packing_proof}

The $\pack$ procedure is given in Algorithm \ref{alg:pack}. 
It can be easily verified that  $\pack$ always returns a feasible assignment $A$ in polynomial time. 

\begin{algorithm}
	\SetAlgoLined
	\SetKwInOut{Input}{Input}\SetKwInOut{Configuration}{Configuration}
	\DontPrintSemicolon
	
	\Input{A set $R\subseteq I$, MKC $(w,B,W)$, a partition $(K_j)_{j=0}^{\ell}$ of the bins to blocks,  $(\bx, \by^0,\ldots, \by^\ell)\in P^e$, where $P^e$ is the extended $\gamma$-polytope of $(K_j)_{j=0}^{\ell}$.}
	\Configuration{$\delta>0$.}

	Initialize $A:B\rightarrow 2^I$ by $A(b) = \emptyset $ for all $b\in B$.\;
	
	Let $I_0,\ldots, I_\ell$ be the Block Association of $((1-\delta)\cdot \bx,  (1-\delta)\cdot\by^0,\ldots, (1-\delta)\cdot\by^{\ell})$  and $\aeps = \frac{\delta }{4}$ (Lemma \ref{lem:association}).
	\label{pack:association} \;
	
	
	\For{$j$ from $0$ to $\ell$ \label{pack:loop}}
	{
		
		\If{$|K_j|>1$}{
		Pack the items in $R\cap I_j$ into bins of capacity $W^*_{K_j}$ using the algorithm of \cite{KK82}. Let $D_1,\ldots, D_{\eta_j}\subseteq I$ be the packing output of the algorithm.\;
	
		Denote $K_j=\{b_1,\ldots, 	b_{|K_j|}\}$\;
		
		Define $A(b_r)= D_r$ for $1\leq r \leq \min\{|K_j|,\eta_j\}$. \;
	}
	\ElseIf{$w(R\cap I_j)\leq W^*_{K_j}$ \label{pack:singleton}}{
		Denote $K_j=\{b\}$ and  set $A(b) = R\cap I_j$. 
	}
	
	}
	Return $A$\;
	\caption{$\pack_{\delta}$} 
	\label{alg:pack}
\end{algorithm}



Let $\eps>0$ and $\delta \in (0,0.1)$.   Let $\rho>0$ be a constant such that the algorithm of \cite{KK82} returns a bin packing using $\OPT+\rho \log^2\OPT$ bins for every bin packing instance. Also, denote $\aeps=  \frac{\delta}{4}$.

By the monotone convergence theorem it holds that 
$$\lim_{N\rightarrow \infty}\sum_{j=1}^{\infty} N^2 \left( 16 \cdot \delta^{-2 } + 2 \right)\cdot\exp  \left(    -\frac{\delta^4}{640}   \cdot N^j \right)=0.$$
Thus there is  $N'_{\eps, \delta}$ such that for any $N>N'_{\eps,\delta}$ it holds that 
$
-\frac{\aeps}{2}N + 4 \cdot 4^{\aeps^{-2}} + 2  + \rho \log^2 N \leq 0 $, $N> 16 \cdot \delta^{-2}$ 
and 
\begin{equation}
\label{eq:N} \sum_{j=1}^{\infty} N^2 \left( 16 \cdot \delta^{-2 } + 2 \right)\cdot\exp  \left(    -\frac{\delta^4}{640}   \cdot N^j \right)< \frac{\eps}{2}.
\end{equation}

Let $N> N'_{\eps,\delta}$, define $\gamma_{\eps, \delta, N}\in \left(0, \frac{\delta}{4} \right)$  such that  for any $0\leq \gamma<\gamma_{\eps, \delta ,N}$ it holds that
\begin{equation}
\label{eq:gamma}
N^2 \exp\left(-\frac{\delta^3}{160} \gamma^{-1} \right)<\frac{\eps}{2}.
\end{equation}

Let $(w,B,W)$  be an  MKC, $(K_j)_{j=0}^{\ell}$  be an $N$-leveled partition of $B$ to blocks for $N\geq N'_{\eps, \delta}$, $\II$  be a valid constraint $\II$, and $(\bx, \by^0,\ldots, \by^{\ell})\in P^e$, where $P^e$ is the extended $\gamma$-partition polytope of $(w,B,W)$ and $(K_j)_{j=0}^{\ell}$ for some $\gamma<\gamma_{\eps,\delta,N}$. 
Furthermore, Let $R$ be a random set sampled by $\bx$, $\delta$ and $\II$, and let $A$ be the output of $\pack_{\delta}$ with the above input. 


For any  $0\leq j \leq \ell$ let $G^j_1,\ldots, G^j_{\tau_j}$ be the $\aeps$-grouping of $(1-\delta)\by^j$ (Definition \ref{def:partition}). 
We define an event $\Psi_j$ for $0\leq j \leq \ell$. For $0\leq j \leq \min\{\ell, N^2-1\}$ (i.e, $|K_j|=1$) define $\Psi_j=\{ w(R\cap I_j)\leq W^*_{K_j}\}$. For $N^2\leq j \leq \ell$ we define
$$\Psi_j=\left\{
\begin{array}{c}\displaystyle \forall 1\leq k \leq \tau_j:~ |R\cap G^j_k \cap I_j|\leq \aeps |K_j|  \textnormal{ and } \\ 
\\
\displaystyle w(R\cap I_j \cap L_{K_j,\aeps}) \leq \sum_{i\in L_{K_j, \aeps} } (1-\delta)\by^j_i \cdot w(i) + \frac{\aeps}{4} W^*_{K_j}\cdot |K_j| 
\end{array}
\right\},$$
where $I_0,\ldots ,I_\ell$ is the Block Association of $(1-\delta)\cdot \bx ,(1-\delta)\cdot \by^0,\ldots, (1-\delta)\cdot \by^{\ell}$, as in Algorithm \ref{alg:pack}.

The lemma follows immediately from the following two claims. 
\begin{claim}
	\label{claim:psi_suff}
If $\Psi_j$ occurs for all $0\leq j \leq \ell$ then $\bigcup_{b\in B} A(b) = R$.
\end{claim}
\begin{proof}
 For any $0\leq j\leq \min\{N^2-1, \ell\}$ it holds that  $|K_j| =1$. Hence, following  iteration $j$ of Step \ref{pack:loop} it holds that $\bigcup_{b\in K_j}A(b) = R\cap I_j$ since the condition in Step \ref{pack:singleton} holds if  $\Psi_j$ occurs. 
 
For any $N^2\leq j \leq \ell$ it holds that $|K_j|\geq N >N'_{\eps, \delta}$.
By Lemma \ref{lem:second_creteria}, as $\Psi_j$ occurs, it follows that $R\cap I_j$ can be packed into at most
$$ (1-\aeps)|K_j| + 4 \cdot 4^{\aeps^{-2}} + 2 + 2 \cdot \frac{\aeps}{4} |K_j|=\left(1-\frac{\aeps}{2}\right)|K_j| + 4 \cdot 4^{\aeps^{-2}} + 2\leq |K_j|$$ 
bins of capacity $W^*_{K_j}$. Therefore, 
$$\eta_j \leq  (1-\aeps)|K_j| + 4 \cdot 4^{\aeps^{-2}} + 2 + 2 \cdot \frac{\aeps}{4} |K_j| + \rho \log^2 |K_j| \leq |K_j|.$$
Hence, following this iteration $j$ of Step \ref{pack:loop} it holds that $\bigcup_{b\in K_j}A(b) = R\cap I_j$. 

Therefore, $\bigcup_{b\in B} A(b)= \bigcup_{j=0}^{\ell}\bigcup_{b\in K_j} A(b) =\bigcup_{j=0}^{\ell} R\cap I_j= R$ where the last equality holds since $R\subseteq \supp(\bx)$ and $I_0,\ldots, I_{\ell}$ is a partition of $\supp(\bx)$.
\end{proof}

\begin{claim}
	\label{claim:psi_prob}
$$
\Pr\left( \forall 1\leq j \leq \ell :~\Psi_j\right)>1-\eps$$
\end{claim}
\begin{proof}

For $0\leq j\leq \min\{N^2-1, \ell\}$, 
by Lemma \ref{lem:association} it holds that there is $i^*\in I$ such that 
$$\sum_{i\in I_j\setminus \{i^*\}} (1-\delta) \bx_i \cdot w(i) \leq \sum_{i\in I} (1-\delta)\by^j_i \cdot w(i)\leq (1-\delta) W^*_{K_j}.$$ Since $\Pr(i\in R )=(1-\delta)^2 \bx_i$ for any $i\in I$, it follows that
$$\E\left[ w(R\cap I_j\setminus \{i^*\}) \right] 
= \sum_{i\in I_j\setminus \{i^*\}} (1-\delta)^2 \bx \cdot w(i )\leq (1-\delta)^2 W^*_k.$$
As $I_j \subseteq \supp\{\by^j\}\subseteq \{i\in I ~|~w(i)\leq \gamma \cdot W^*_{K_j}\}$ (see \eqref{eq:gamma_partition}), and $\gamma<\frac{\delta}{2}$ it follows that
$\E\left[ w(R\cap I_j) \right]  \leq \left(1-\frac{\delta}{2}\right)\cdot W^*_{K_j}$. Hence,
$\E\left[ \sum_{i\in R} \frac{\one_{i\in I_j} \cdot w(i)}{\gamma\cdot W^*_{K_j}} \right]  \leq \left(1-\frac{\delta}{2}\right)\cdot \frac{1}{\gamma}$.
 \footnote{For $i\in I$ and $S\subseteq I$ we use $\one_{i\in S}=1$ if $i\in s$ and $\one_{i\in S}=0$ otherwise.} Following the same argument and by Lemma \ref{lem:sampling} it holds that
\begin{equation}
\label{eq:psi_singlton}
\begin{aligned}
\Pr&(\neg \Psi_j) = \Pr( w(R\cap I_j) >W^*_{K_j}) =
\Pr\left(\sum_{i\in R} \frac{\one_{i\in I_j} \cdot w(i)}{\gamma\cdot W^*_{K_j}} >\gamma^{-1} \right)
\\&
\leq Pr\left(\sum_{i\in R} \frac{\one_{i\in I_j} \cdot w(i)}{\gamma\cdot W^*_{K_j}} \geq \left( 1+\frac{\delta}{2}\right)\left(1-\frac{\delta}{2}\right)\cdot \frac{1}{\gamma} \right)
%\\&
\leq 
\exp\left( -\frac{\delta^3}{80}
\left(1-\frac{\delta}{2}\right)\cdot \gamma^{-1}
\right)
\\&
 \leq \exp\left( -\frac{\delta^3}{160}
\cdot \gamma^{-1}
\right)
\end{aligned}
\end{equation}

For $N^2\leq  j \leq \ell$, by Lemmas \ref{lem:association}  and \ref{lem:sampling} for any $1\leq k \leq \tau_j$ it holds that
$$\E\left[ |R\cap I_j \cap G^j_k|  \right] \leq (1-\delta )\left(\aeps |K_j| +2 \right)\leq \left( 1-\frac{\delta}{2}\right)\aeps |K_j|,$$
where the last transition holds since $|K_j|>N'_{\eps,\delta}$ and thus $|K_j| >16\cdot\delta^{-2} =4\cdot \delta^{-1}  \cdot \aeps^{-1}$. 
Hence, following Lemma \ref{lem:sampling} it holds that
\begin{equation}
\label{eq:partition_prob}
\begin{aligned}
\Pr&\left( |R\cap I_j \cap G^j_k|>\aeps |K| \right)
\leq
\Pr\left( \sum_{i\in R} \one_{i\in I_j\cap G^j_k} \geq \left(1+\frac{\delta}{2}\right) \left( 1-\frac{\delta}{2}\right)\aeps |K_j|\right)\\
&\leq  \exp\left(-\frac{\delta^3}{80} \cdot\left(1- \frac{\delta}{2}\right) \aeps |K_j|\right) = \exp\left(-\frac{\delta^4}{640}\cdot   |K_j|\right)
\end{aligned}
\end{equation}
Similarly, by Lemma \ref{lem:association} there is $i^*\in I$ such that $\sum_{i\in I_j \cap L_{K_j, \aeps} \setminus \{i^*\}} (1-\delta) \bx_i \cdot w(i) \leq \sum_{i\in L_{K_j, \aeps}} (1-\delta) \by^j_i \cdot w(i)$. Thus, $$\sum_{i\in I_j \cap L_{K_j, \aeps} } (1-\delta) \bx_i \cdot w(i) \leq \sum_{i\in L_{K_j, \aeps}} (1-\delta) \by^j_i \cdot w(i) +\aeps W^*_{K_j} \leq 
 \sum_{i\in L_{K_j, \aeps}} (1-\delta) \by^j_i \cdot w(i) +\frac{\aeps}{4} |K_j| W^*_{K_j},$$
 where the last transition requires $|K_j|\geq 4$ which  holds due to the parameter selection. Let $\zeta  = \sum_{i\in L_{K_j, \aeps}} (1-\delta) \by^j_i \cdot w(i) +\frac{\aeps}{4}\cdot |K_j| \cdot W^*_{K_j}$. Subsequently, by Lemma \ref{lem:sampling} we have $\E\left[ w(I_j\cap L_{K_j,\aeps} \cap R)\right] \leq (1-\delta)\zeta$ and 
 \begin{equation}
 \label{eq:slack_prob}
 \begin{aligned}
 \Pr&\left(  w(I_j \cap L_{K_j, \aeps} \cap R) > \zeta\right) \leq  \Pr \left( \sum_{i\in R} \one_{i\in I_j \cap L_{K_j, \aeps }} \cdot \frac{w(i)}{W^*_{K_j}} \geq (1+\delta)(1-\delta )\frac{\zeta}{W^*_{K_j}} \right)\\
&\leq \exp  \left(    -\frac{\delta^3}{20} \cdot (1-\delta) \cdot  \frac{\zeta}{W^*_{K_j}} \right)\leq 
\exp  \left(    -\frac{\delta^4}{640}   \cdot  |K_j| \right).
 \end{aligned}
 \end{equation}
 The last inequality used $\zeta \geq \frac{\aeps}{4} \cdot |K_j| \cdot W^*_{K_j}= \frac{\delta}{16} \cdot |K_j| \cdot W^*_{K_j}$.
 By \eqref{eq:partition_prob} and \eqref{eq:slack_prob}, it follows that 
 \begin{equation}
 \label{eq:psi_multi}
 \begin{aligned}
 \Pr(\neg \Psi_j ) &\leq (1+\tau_j) \exp  \left(    -\frac{\delta^4}{640}   \cdot  |K_j| \right) \leq %(\aeps^{-2}+1)
 % \exp  \left(    -\frac{\delta^4}{320}   \cdot  |K_j| \right) 
 %\\
% &=
 \left(16\cdot \delta^{-2}+2\right) \exp  \left(    -\frac{\delta^4}{640}   \cdot  |K_j| \right),
 \end{aligned}
 \end{equation}
 where the second inequality follows from $\tau_j \leq \aeps^{-2}+1 \leq 16\cdot \delta^{-2}+1$ (Lemma \ref{lem:partition_prop}). 
  
 By \eqref{eq:psi_singlton} and \eqref{eq:psi_multi}, it holds that 
 \begin{equation*}
 \Pr(\exists 0\leq j\leq \ell:~\neg \Psi_j) \leq 
 N^2 \exp\left(-\frac{\delta^3}{160} \gamma^{-1} \right)
 +\sum_{j=1}^{\infty} N^2 \left( 16 \cdot \delta^{-2 } + 2 \right)\cdot\exp  \left(    -\frac{\delta^4}{640}   \cdot N^j \right) <\eps, \end{equation*}
 where the last inequality is by \eqref{eq:gamma} and \eqref{eq:N}. 
The claim follows immediately.
\end{proof}
By Claims \ref{claim:psi_suff} and \ref{claim:psi_prob} it follows that 
$$\Pr\left( \bigcup_{b\in B} A(b)= R \right) \geq \Pr( \forall 1\leq j \leq \ell:~ \Psi_j)>1-\eps.$$
Hence, 
$$\Pr\left( \bigcup_{b\in B} A(b)\neq R \right) =
1- \Pr\left( \bigcup_{b\in B} A(b)= R \right) <\eps.$$
\qed


==> prelim.tex <==
We first define a few technical notations which are used throughout the paper.

Given an MKC instance $(w,B,W)$ over $I$, a subset of bins $K\subseteq B$ is a {\em block} if all the bins in the block have the same capacity, i.e., $W_{b_1}= W_{b_2}$ for every $b_1, b_2\in K$. In particular, in the Submodular Multiple Knapsack Problem with Uniform Capacities the set $B$ of all bins is a block. We use $W^*_K$ to denote the capacities of the bins in  block $K$, that is, $W^*_K=W_b$ for any $b\in K$. 

We say an item $i\in I$ is {\em $\aeps$-heavy} for $\aeps>0$ (w.r.t $K$) if $W^*_K \geq w(i) > \aeps \cdot W^*_K$.
We say $i\in I$ is {\em $\aeps$-light} if $w(i)\leq \aeps\cdot W^*_K$. We use $H_{K,\aeps}$ and $L_{K, \aeps}$  to denote the sets of $\aeps$-heavy items  and $\aeps$-light items respectively. 


Given a subset of items $S\subseteq I$ we use the notation $w(S)=\sum_{i\in S} w(i)$. Given a polytope $P$ and $\delta\in \mathbb{R}$  we use the notation $\delta P = \{\delta \bx ~|~ \bx \in P\}$.  We also use $\one_S=\bx\in \{0,1\}^I$ where $\bx_i = 1$ if $i\in S$ and $\bx_i = 0$ if $i\in I\setminus S$. Similarly, we use $\one_{i\in S}=1$ if $i\in s$ and $\one_{i\in S}=0$ otherwise.

\ariel{I am not sure preliminaries it the right title, and that the section is a good idea}

==> structuring.tex <==

\newcommand{\rlast}{{r_{\textnormal{last}}}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\mL}{\mathcal{L}}

\section{Proof of Lemma \ref{lem:structuring}}
\label{sec:structuring}
In this section we provide a proof for Lemma \ref{lem:structuring}. The proof follows from \cite{FKNRS20} with minor adaptations.


\begin{algorithm}[H]
	\SetAlgoLined
%\SetKwInOut{Configuration}{Configuration}
\SetKwInOut{Input}{Input}\SetKwInOut{Configuration}{Configuration}
%\Configuration{The parameters $N,P, \delta$ and $\mu$.}
%{\bf Input:} 
%\Input{An SMKP instance $\II =(I,w,B,W,f)$.} %$I=\{1,\ldots, n\}$, $(w_i)_{i\in I}$ $B=\{1,\ldots, m\}$, $(W_b)_{b\in B}$, and a monotone submodular function $f$.}
\DontPrintSemicolon

\Input{A set of bins $B$, capacity function  $W:B\rightarrow \mathbb{R}_{\geq 0}$ and $N\in \mathbb{N}$.} 

	
Let $B=\{1,\ldots, m\}$ where $W(1)\geq W(2) \geq \ldots \geq W(m)$.\;

Let $\ell = \max \left\{k \in \mathbb{N} ~\middle|~\sum_{r=0}^{k} N^{\floor{\frac{r}{N^2}}} \leq m\right\}$. \;

Define $\tilde{K}_{j}= \left\{ b~\middle|~
\sum_{r=0}^{j-1} N^{\floor{\frac{r}{N^2}}} ~< ~b~\leq \sum_{r=0}^{j} N^{\floor{\frac{r}{N^2}}} 
\right\}$  for $0\leq j \leq \ell$.\; 

Let $\tilde{B}= \bigcup_{j=0}^\ell \tilde{K}_j$, and $\tilde{W}(b)= \min_{b'\in \tilde{K}_j} W(b')$ for all $0\leq j \leq \ell$ and $b\in \tilde{K}_j$.\;

Return $\tilde{B}$, $(\tilde{W}_b)_{b\in \tilde{B}}$ and the partition $(\tilde{K}_j)_{j=0}^\ell$. 

\caption{Structure in Blocks}
\label{alg:structuring}
\end{algorithm}


By construction, we have that $(\tilde{K}_j)_{j=0}^{\ell}$ is an $N$-leveled partition of  $\tilde{B}$. Furthermore, $\tilde{B}\subseteq B$ and  $\tilde{W}(b) \leq W(b)$ for any $b\in \tilde{B}$. Finally, it can be  easily observed that  Algorithm \ref{alg:structuring} has a polynomial running time. Thus, the following Lemma completes the proof of Lemma \ref{lem:structuring}.


\begin{lemma}
Let $N\in \mathbb{N}$, $B$ be a set of bins, $W:B\rightarrow \mathbb{R}_{\geq 0}$ be a capacity function, and let $\tilde{B}$, $\tilde{W}$ be the output of Algorithm \ref{alg:structuring}  for the input $B$, $W$ and $N$.
 Furthermore, let $I$ be a set of items, $w:I\rightarrow \mathbb{R}_{\geq 0}$ a weight function, $S\subseteq I$ feasible for $(w,B,W)$ and $f:2^I \rightarrow \mathbb{R}_{\geq 0}$ submodular non-negative function. Then there is $\tilde{S}\subseteq S$ feasible for $(w,\tilde{B}, \tilde{W})$ such that $f(\tilde{S})\geq \left( 1- \frac{1}{N}\right)f(S)$.
\end{lemma}
\begin{proof}

W.l.o.g assume $B=\{1,2,\ldots, m\}$ and $W(1)\geq W(2)\geq \ldots \geq W(m)$. 
 Let  $A$ be a feasible disjoint  assignment of $S$ w.r.t. the MKC $(w,B,W)$.
 We modify this assignment using a sequence of steps, eventually obtaining a feasible assignment of a set $\tilde{S}\subseteq S$ with respect to $(w,\tilde{B}, \tilde{W})$ . 
 
 Define $\tilde{K}_{\ell+1} = B\setminus \tilde{B}$. We note that  $\tilde{K}_{\ell+1}$ may be empty. We partition $\{\tilde{K}_j|~ 0\leq j \leq \ell+1\}$ into {\em levels} and {\em super-bloks}. We consider each $N^2$ consecutive blocks to be a {\em level}, and each $N$ consecutive blocks within a level to be a {\em super-block}. Formally, level $t$ is
$$\mL_t =\left\{j~| ~t\cdot N^2 \leq j <\min\{(t+1)N^2, ~\ell+2 \}\right\}$$ 
for $0\leq t \leq k$ with $k = \floor{\frac{\ell+1}{N^2}}$. Also, super-block 
$r$ of level $t$ is  
$$\mS_{t,r} = \left\{j~|~ t\cdot N^2 +r\cdot N\leq j  < t\cdot N^2 +(r+1)\cdot N \right\}$$
 for $0\leq r<N$ and level $0\leq t <k$ (we do not partition the last level into super-blocks). 
 It  follows that ${B}= \bigcup_{t=0}^{k} \bigcup_{j\in \mL_t} \tilde{K}_j$ and $\mL_t=\bigcup_{r=0}^{N -1 } \mS_{t,r}$ for $0\leq t<k$. Furthermore, for any $j\in \mL_t$, $j\neq \ell+1$  it holds that $|\tilde{K}_j| =N^t$ and $|\tilde{K}_{\ell+1}| < N^{\ell}$. Essentially, all the blocks of level $t$ are of the same size. 
%
%Each super-block consist of $N$ consecutive blocks and each level level consist of $N$ consecutive super-blocks, with a possible exception in the last level and last block.
%Formally, let 
%
%Let $\ell,k$ be the maximal values (lexicographically) such that $B\cap B_{\ell ,k} \neq \emptyset$. We refer to $\ell$ as the last level.  We use the term block to refer to the bins in $B_{t,j}$ for some $t$ and $j$, even though it is not formally a block with respect to $W_1,\ldots, W_m$. Similarly, we use the term level to refer to a the  blocks $(B_{t,j})_{1\leq j \leq N^2}$ for a some $t\geq 0$. The alternation steps are as follows (we ignore some handling of corner cases in this sketch).

We note that if $k=0$, then $A$ is a feasible assignment w.r.t $(w,\tilde{B},\tilde{W})$ and the claim hold. Thus, we can assume that $k\geq 1$. We modify the assignment  $A$ using the following steps. 

%\begin{enumerate}
%	\item  
\noindent	{\bf Eviction: }
		We first evict a super-block of bins from each level (except the last one). Let $R= \bigcup_{b\in \mL_{k}} A(b)$ be the subset of items assigned to the last level and let $g:2^I \rightarrow \mathbb{R}_{\geq 0}$ defined by $g(Q) = f(Q \cup R)$.
	%\begin{equation*}
	%f\left(A^*\right) = f_R\left( \bigcup_{t=0}^{\ell-1}\bigcup_{r=0}^{N-1} \bigcup_{~j\in \mS_{t,r}~} \bigcup_{b\in \tilde{B}_j}  A^*_b\right)+f(R).
	%\end{equation*}
	As $g$ is submodular and non-negative (Lemma \ref{lem:submodular_cup}),
	by Lemma \ref{lem:submodular_evict} for every $0\leq t <k$ there is $r^*_t$ such that 
	\begin{equation*}
	\begin{aligned}
	g&\left(  \bigcup_{t=0}^{k-1}\bigcup_{
		~0\leq r < N, ~r\neq r^*_t
} \bigcup_{~j\in \mS_{t,r}} \bigcup_{~b\in \tilde{K}_j}  A(b)\right) %\\
%	&
	\geq 
	 \left(
	 %\frac{N-1}{N}
	  1-\frac{1}{N}
	 \right)
	 g\left( \bigcup_{t=0}^{k-1}\bigcup_{r=0}^{N-1} \bigcup_{~j\in \mS_{t,r}} \bigcup_{~b\in \tilde{K}_j} A(b)\right)   
	 =
	  \left( 1-\frac{1}{N}\right) f(S).
	\end{aligned}
	\end{equation*}
	
	Define $T:B\rightarrow 2^I$  by $T(b) = \emptyset$ 
	for any  $b\in \bigcup_{t=0}^{k -1} \bigcup_{~j\in \mS_{t,r^*_t} }\tilde{K}_j$, 
	and $T(b) = A(b)$ for any  $b\in B \setminus \left( \bigcup_{t=0}^{k -1} \bigcup_{~j\in \mS_{t,r^*_t} }\tilde{K}_j\right)$. Also, denote $\tilde{S}= \bigcup_{b\in B} T(b)\subseteq S$.  Then,
	\begin{equation}
	\label{eq:tilde_S_lb}
	f(\tilde{S})=f\left(\bigcup_{b\in B} T(b)\right) =
	g\left(  \bigcup_{t=0}^{k-1}\bigcup_{~0\leq r < N-1,~r\neq r^*_t~} \bigcup_{j\in \mS_{t,r}} \bigcup_{b\in \tilde{K}_j}  A(b)\right)
	\geq  \left( 1-\frac{1}{N}\right) f(S).
	\end{equation}
	It also holds that $T$ is a feasible assignment  with respect to  $(w,B,W)$ as $T(b)\in \{ A(b), \emptyset\}$ for any $b\in B$. 
	
	

 	 \noindent {\bf Shuffling:} We generate a new assignment $\tilde{T}$ such that $\bigcup_{b\in B} \tilde{T}(b) = \bigcup_{b\in B} T(b)$ and the last super-block in each level (except the last one) is empty. 
 	 This property is obtained by moving the assignments of
 	 the  bins in  super-block $N-1$ to the bins of super-block $r^*_t$ for every $0\leq t <k$. 
 	 
 	 We define $\tilde{T}:B\rightarrow 2^I$ as follows.
 	 For any $0\leq t<k$, 
 	 let $\varphi_t:\bigcup_{j\in \mS_{t,r^*_t}} \tilde{K}_j \rightarrow 
 	 \bigcup_{j\in \mS_{t,N-1}} \tilde{K}_j $ be a bijection between the bins of super-block $r^*_t$ to the bins of the last super-block of level $t$ (note that both sets have the same cardinality, thus such a bijection exists). 
	For any $0\leq t<k$, 
 	 $j\in \mS_{t,r^*_t}$,
 	  and $b\in \tilde{K}_j$, define $\tilde{T}(b) = T(\varphi_t(b))$. In this case, it holds that $$w(\tilde{T}(b)) \leq w(T(\varphi_t(b))) \leq W(\varphi_t(b)) \leq W(b)$$
 	  where the last inequality follows from $\varphi_t(b)\geq b$.  
 	 This step defines the assignment of the last super-block in place of super block $r^*_t$ for every $0\leq t< k$.
 	  For every $0\leq t<k$, $j\in \mS_{t,N-1}$ and $b\in \tilde{K}_j$ define $\tilde{T}({b}) =\emptyset$. 
 	 For any other bin $b\in B$ define $\tilde{T}(b) = T(b)$. 
 	 
 	 It follows that $\bigcup_{b\in B} \tilde{T}(b) = \bigcup_{b\in B} T(b)$, since $T(b)= \emptyset$ for every $0\leq t<k$, $j\in \mS_{t,r^*_t}$ and $b\in \tilde{K}_j$. Also, it holds that $\tilde{T}$ is a feasible assignment w.r.t $(w,B,W)$.
 	 %s $N^2 - N+1,\ldots , N^2$  to the bins in blocks $N(r^*_t-1) +1,\ldots, N\cdot r^*_t$. As the latter are empty due to the previous step, this will not change the set of items in the solution. Also, since the bins are ordered by decreasing capacities, the capacity constraints are preserved.
 	 %\item 
 	 
 	 
 	 \noindent{\bf Shifting:}
 	  In this step we generate an assignment $\tilde{A}$ of $\tilde{S}$ such that $\tilde{A}$ is feasible with respect to $(w,\tilde{B}, \tilde{W})$. 
 	  As the bins of the last super-block in each level (except the last level)  are vacant in $\tilde{T}$, we use them for the assignment of the first block of the next level.
 	  This can be done 
 	 since $N$ blocks of level $t$ contain the same number of bins as a single block of level $t+1$. We also use blocks in levels greater than $0$ which are not in the last  super-block to store the assignment of the subsequent block in the level. 
 	 
 	 Formally, define $\tilde{A}(b-N^t)= \tilde{T}(b)$ for any $b\in \bigcup_{t=1}^{k -1 } \bigcup_{j\in \mL_t\setminus \mS_{t,N-1} } \tilde{K}_j$. 
 	  Define $\tilde{A}(b-N^{k})=\tilde{T}(b)$ for any $b\in \bigcup_{j \in \mL_k} \tilde{K}_j$.  Also,  define $\tilde{A}(b)=\tilde{T}(b)$ for %$b\in \mL_0$ and 
 	  $0\leq b \leq N^2 -N$. For any bin $b\in \tilde{B}$ which was not defined above, set $\tilde{A}(b)= \emptyset$. 
 	 It can be easily verified that for any $t\geq 0$, $j \in \mL_t$ and $b\in \tilde{K}_j$, if $j>t\cdot N^2$ (i.e., not the first block in the level) then  $b-N^t \in \tilde{K}_{j-1}$ and $b-N^t\in \bigcup_{j'\in \mS_{t-1, N-1} }\tilde{B}_j$ if $j=t\cdot N^t$. This implies that the definition of $(A_b)_{b\in \tilde{B}}$ is sound. 
 	 
 	Let $b\in \tilde{B}$. If $b\leq N^2-N$ then
 	 it holds that $\tilde{K}_{b-1} = \{b\}$. Therefore, $w(\tilde{A}(b))= w(\tilde{T}(b)) \leq W(b)= \tilde{W}(b)$. 
 	 Also, if $\tilde{A}(b)=\emptyset$ then $w(\tilde{A}(b))=0\leq \tilde{W}(b)$. 
 	 In all other cases, $b\geq N^2 -N$ for
 	  $b\in \tilde{K}_j$, 
 	  and it holds that $\tilde{A}(b)= \tilde{T}(b')$ for $b'\in \tilde{K}_{j'}$ with $j'>j$.
 	  Since the capacities are assumed to be sorted, for any $c\in \tilde{K}_j$ it holds that $W(c)\geq W(b')$. Thus, $\tilde{W}(b) \geq W(b')$ and 
 	   $w(\tilde{A}(b)) =w(\tilde{T}({b'})) \leq W(b') \leq \tilde{W}(b)$.  Overall, we have that $\tilde{A}$ is a feasible solution w.r.t. $(w,\tilde{B},\tilde{W})$. Furthermore, it holds that $\bigcup_{b\in \tilde{B}} A(b) = \bigcup_{b\in B} \tilde{T}(b)= \bigcup_{b\in B} T(b)=\tilde{S}$.
 	
 	
 	That is, we showed that $\tilde{S}\subseteq S$ is feasible for $(w,\tilde{B} , \tilde{W})$ and $f(\tilde{S}) \geq \left( 1- \frac{1}{N} \right) f(S)$, therefore proving the lemma.

\end{proof}




%A complete and formal proof of Lemma \ref{lem:structuring} is provided in Appendix \ref{app:gT_bound}.

%  \begin{algorithm}[H]
% \SetAlgoLined
% \DontPrintSemicolon
% $i=0$ \;
% \While {$B\neq\emptyset$} {
%     \For{$j=1,...,\delta^{-2}$}{
%         \If{$|B|<\delta^{-i}$}{
%             $W^*_b = 0, \forall b\in B$. \;
%             $L_i = L_i\cup\{B\}$. \;
%             $B=\emptyset$. \;
%         }
%         \Else{
%             Let $T$ be the largest $\delta^{-i}$ bins. \;
%             $B^i_j = T, ~~B = B\setminus T$. \;
%             $W^*_b = \min_{b'\in B^i_j}W_{b'}, \forall b\in B^i_j$. \label{equal-capacities} \;
%             $L_i = L_i \cup \{B^i_j\}$. \;
%             $i = i+1$ \;
%         }
%     }
%     Return $W^*$.
